Guarantees for Comprehensive Simulation Assessment of Statistical Methods

Simulation can evaluate a statistical method for properties such as Type I Error, FDR, or bias on a grid of hypothesized parameter values. But what about the gaps between the grid-points? Continuous Simulation Extension (CSE) is a proof-by-simulation framework which can supplement simulations with (1) confidence bands valid over regions of parameter space or (2) calibration of rejection thresholds to provide rigorous proof of strong Type I Error control. CSE extends simulation estimates at grid-points into bounds over nearby space using a model shift bound related to the Renyi divergence, which we analyze for models in exponential family or canonical GLM form. CSE can work with adaptive sampling, nuisance parameters, administrative censoring, multiple arms, multiple testing, Bayesian randomization, Bayesian decision-making, and inference algorithms of arbitrary complexity. As a case study, we calibrate for strong Type I Error control a Phase II/III Bayesian selection design with 4 unknown statistical parameters. Potential applications include calibration of new statistical procedures or streamlining regulatory review of adaptive trial designs. Our open-source software implementation imprint is available athttps://github.com/Confirm-Solutions/imprint

==> archive/experimental.tex <==
% List results that are experimental and need deliberation of adding into main.
% It's still useful to keep some of these results around
% even if we don't ever put them in main.
% But this will definitely help clean-up main.tex so that it always has
% content that we want to publish.

\section{Experimental Results}

\begin{theorem}[O-net]\label{thm:main-o-net}
Let $\set{P_{\theta} : \theta \in H}$ be a 
family of distributions, where
$H \subseteq \R^d$ is a tile with an associated grid point
$\theta_0 \in \R^d$.
Let $x \mapsto F(x)$ have range in $[0,1]$.
Define $f(\theta) := \EEE_\theta[F(X)]$
where $X \sim P_{\theta}$. 
Further assume that for every $\theta, \theta' \in H$,
$P_{\theta}$ is absolutely continuous with respect to $P_{\theta'}$,
and $F$ is not trivially $0$ or $1$ ($P_\theta$-a.e. for all $\theta \in H$).
Additionally, assume that $\forall \theta \in H$,
\begin{align}
    \nabla \int F(x) p_{\theta} d\mu(x)
    =
    \int F(x) \nabla p_{\theta} d\mu(x). \label{eq:interchange}
\end{align}
Let $X_1,\ldots, X_n \sim P_{\theta_0}$ be
i.i.d. samples.
Fix any $\delta \in [0,1]$.
Then, for any estimate $\hat{f}(\theta_0)$
using the samples $X_1,\ldots, X_n$ such that
\[
\prob\br{f(\theta_0) \leq \hat{f}(\theta_0)} \geq 1-\delta
\]
there exists a random function $\hat{U}(\theta) : H \mapsto \R$ such that
\begin{align*}
    \prob\br{f(\theta) < \hat{U}(\theta) }
    &\geq
    1-\delta,
    \quad \forall \theta \in H.
\end{align*}
Moreover, for any $q \geq 1$, $c \in [0,1]\backslash \set{0.5}$,
this property is achieved by the random function
\begin{align*}
    \hat{U}^c_q(\theta) 
    &:= 
    \frac{1}{A}\pr{\frac{AC_q}{q} + (A\hat{f}(\theta_0)+ B)^{\frac{1}{q}}}^q - \frac{B}{A}
\end{align*}
where
\begin{align*}
    C_q 
    := 
    C_{q}(\theta_0, H) 
    &:=
    \sup\limits_{v \in H-\theta_0}
    \int_0^1
    \norm{
        \frac{d}{dh} \log p_{\theta_0 + hv}(X)
    }_{L^q(P_{\theta_0+hv})}
    dh
    \\ p & := \frac{q}{q - 1} 
    \\ A & := (1 - c)^p - c^p, 
    \\ B & := c^p
\end{align*}

\end{theorem}

\begin{proof}

Fix any $v \in H-\theta_0$.
We begin with the directional derivative, defining
\[g(h) := f(\theta_0 + hv)\]
By differentiating $g$ and applying H\"{o}lder's Inequality for any conjugate $p, q > 1$, we find that for any $c \in [0,1]\backslash\set{0.5}$,
\begin{align}
    g'(h)
    &=
    \nabla f(\theta_0 + hv)^\top v
    =
    \EEE_{\theta_0 + hv}\br{
        F(X) \frac{d}{dh} \log p_{\theta_0+hv}(X)
    }
    \\&= 
    \EEE_{\theta_0 + hv}\br{
        (F(X) - c) \frac{d}{dh} \log p_{\theta_0+hv}(X)
    } \label{eq:introduce-c}
    \\&\leq
    \norm{F(X) - c}_{L^p(P_{\theta_0+hv})}
    \norm{
        \frac{d}{dh} \log p_{\theta_0 + hv}(X)
    }_{L^q(P_{\theta_0+hv})}
    \\&\leq
    |((1-c)^p - c^p) g(h) + c^p |^{\frac{1}{p}}
    \norm{
        \frac{d}{dh} \log p_{\theta_0 + hv}(X)
    }_{L^q(P_{\theta_0+hv})} \label{eq:substitute-lemma}
\end{align}
where (\ref{eq:introduce-c}) is implied by
assumption~(\ref{eq:interchange}), which requires that 
\begin{align*}
    \EEE_{\theta}\br{\nabla_\theta \log p_{\theta}(X)} &= 0 
    \quad \forall \theta \in H
    \\\implies
    \EEE_{\theta_0+hv}\br{\frac{d}{dh} \log p_{\theta_0+hv}(X)} &= 0 
    \quad \forall h \in [0,1]
\end{align*}
and (\ref{eq:substitute-lemma}) is an application of 
Lemma~\ref{lemma:holdernonsense}. 
The result (\ref{eq:substitute-lemma}) is 
an Ordinary Differential Inequality (ODI).
Note that by assumption and Lemma~\ref{lem:common-support},
we have that $g \in (0,1)$.
Since $c$ lies in $[0,1]$ as well, 
we have that $((1-c)^p - c^p) g(h) + c^p > 0$. 
We may then solve this ODI:
\begin{align}
    \int_{0}^t g'(h) (((1-c)^p - c^p) g(h) + c^p ))^{-\frac{1}{p}} dh
    \leq
    \int_0^t 
    \norm{
        \frac{d}{dh} \log p_{\theta_0 + hv}(X)
    }_{L^q(P_{\theta_0+hv})}
    dh
\end{align}
The left side evaluates to
\begin{equation}
    \frac{q}{(1-c)^p - c^p }\br{ (((1-c)^p - c^p) g(t) + c^p)^{\frac{1}{q}} - (((1-c)^p - c^p) g(0) + c^p)^{\frac{1}{q}}}
    %\leq
    %\int_0^t 
    %\norm{
    %    \frac{d}{dh} \log p_{\theta_0 + hv}(X)
    %}_{L^q(P_{\theta_0+hv})}
    %dh
\end{equation}
Then, abbreviating with constants $A:= (1-c)^p - c^p$ and $B := c^p$, we have
\begin{equation}
  \implies
    g(t) 
    \leq \frac{1}{A}
    \pr{
        \frac{A}{q}
        \int_0^t
        \norm{
            \frac{d}{dh} \log p_{\theta_0 + hv}(X)
        }_{L^q(P_{\theta_0+hv})} dh
        +
        (A g(0) + B)^{\frac{1}{q}}
    }^q - \frac{B}{A}
\end{equation}
In particular, we have that
{\small
\begin{align}
    f(\theta_0 + v)
    &\leq
    \frac{1}{A}
    \pr{
        \frac{A}{q}
        \int_0^1
        \norm{
            \frac{d}{dh} \log p_{\theta_0 + hv}(X)
        }_{L^q(P_{\theta_0+hv})}
        dh
        +
        (Af(\theta_0) +B)^{\frac{1}{q}}
    }^q - \frac{B}{A}
    \label{eq:main-o-net:odi-sol}
\end{align}
}
Hence, defining $C_q$ as in the theorem statement,
\begin{align}
    \sup\limits_{\theta \in H}
    f(\theta)
    &\leq
   \frac{1}{A}
    \pr{
        \frac{A C_q}{q}
        +
        (Af(\theta_0) +B)^{\frac{1}{q}}
    }^q - \frac{B}{A}
    \label{eq:main-o-net:odi-fullsolved}
\end{align}

The remainder of the proof follows directly.
Let $\hat{f}(\theta_0)$ be any estimate
using the data $X_1,\ldots, X_n$ such that
\[
\prob\br{f(\theta_0) \leq \hat{f}(\theta_0) } \geq 1 - \delta
\]
Let $\hat{U}(\theta)$ be defined as in the
theorem statement.
Then, for any $\theta \in H$,
\begin{align*}
    \prob\br{f(\theta) \leq \hat{U}(\theta)}
    &\geq
    \prob\br{\sup\limits_{\theta \in H} f(\theta)\leq \hat{U}(\theta) }
    \geq
    \prob\br{f(\theta_0) \leq \hat{f}(\theta_0)}
    \geq
    1 - \delta
\end{align*}

\end{proof}

\begin{lemma}
\label{lemma:holdernonsense}

For any random variable $X$ on $\mathbbm{X}$ with probability distribution $Q$, $F$ any function $F(
\cdot) : \mathbbm{X} \rightarrow [0,1]$ and $c$ a scalar $\in [0,1]$, and $p \geq 1$

$$ \|F(X) - c \|^p_{L^p(Q)} \leq E_{Q}[F(X)] ((1-c)^p - c^p)  + c^p $$

\begin{proof}
    We begin with the simple inequality
    for any $a \in [0,1]$:
    \begin{equation}
        |a-c|^p \leq a(|1-c|^p - |c|^p ) + |c|^p \label{eq:simpleinequality}
    \end{equation}
 
    This follows by convexity, since equality holds at $a = 0$ and $a = 1$, the right side is linear in $a$, and the left side is convex in $a$. Lemma \ref{lemma:holdernonsense} then follows by replacing $a$ in (\ref{eq:simpleinequality}) with $F(X)$, and integrating over $Q$.
\end{proof}

\begin{lemma}\label{lem:common-support}
    Let $\set{P_\theta : \theta \in \Theta}$ be a family of distributions
    for any set $\Theta$.
    Let $x \mapsto F(x)$ be any measurable function 
    whose range is in $[0,1]$.
    Assume that $P_\theta$ is absolutely continuous with respect to
    $P_{\theta'}$ for all $\theta, \theta' \in \Theta$.
    If $\EEE_\theta\br{F(X)} = c \in \set{0,1}$ for some $\theta$,
    then $F(x) = c$ $P_\theta$-a.s. for every $\theta$.
\end{lemma}
\begin{proof}
    Without loss of generality, assume that
    $\EEE_\theta\br{F(X)} = 0$ for some $\theta$.
    The proof for when it is equal to $1$ is identical
    by considering $1-F(x)$.
    Then, $F(x) = 0$, $P_\theta$-a.s.
    Let $A := \set{x : F(x) = 0}$.
    Then, for any $\theta' \in \Theta$,
    by Radon-Nykodym Theorem,
    \begin{align*}
        \prob_{\theta'}\br{A}
        &=
        \EEE_{\theta'}\br{\indic{A}(X)}
        =
        \EEE_{\theta}\br{\indic{A}(X) \frac{dP_{\theta'}}{dP_\theta}(X)}
        =
        \EEE_{\theta}\br{\frac{dP_{\theta'}}{dP_\theta}(X)}
        =
        1
    \end{align*}
\end{proof}

\begin{remark}
Exponential families and log-concave distributions with the same base measure
all satisfy the conditions of Lemma~\ref{lem:common-support}.
Consequently, if the true Type I Error of a design is 0 or 1
under some distribution in the family, 
it must be 0 or 1, respectively, under any distribution in the family.
Hence, we may safely assume without loss of generality
that the true Type I Error is in the range $(0,1)$ to avoid trivialities.
\end{remark}

\end{lemma}

\begin{corollary}[\bf A Practical Simplification]\label{cor:main-o-net} 
Consider the setting of Theorem~\ref{thm:main-o-net}.
Then, we may conservatively replace $C_q$ with the following $C_q'$:
\begin{align*}
    C_q' := \sup\limits_{v \in H-\theta_0} \norm{v}_{l^p}
    \cdot
    \sup\limits_{\theta \in H} 
    \norm{\norm{
    \nabla \log p_{\theta}(X)
    }_{l^q}}_{L^q(P_\theta)}
\end{align*}
to achieve the same conclusions as Theorem~\ref{thm:main-o-net}.
\end{corollary}

\begin{proof}
Consider $C_q$ as defined in Theorem~\ref{thm:main-o-net}.
Let 
\begin{align*}
    s_v(h, X) 
    &:= 
    \frac{d}{dh} \log p_{\theta_0 + hv}(X)
    \\&=
    \nabla \log p_{\theta_0 + hv}(X)^\top v
    \\\implies
    \abs{s_v(h, X)}
    &\leq
    \norm{\nabla \log p_{\theta_0 + hv}(X)}_{l^q}
    \norm{v}_{l^p}
\end{align*}
Then,
\begin{align*}
    &\sup\limits_{v \in H-\theta_0}
    \sup\limits_{h \in [0,1]}
    \norm{
        s_v(h, X)
    }_{L^q(P_{\theta_0+hv})}
    \\&\qquad \leq
    \sup\limits_{v \in H-\theta_0} \norm{v}_{l^p}
    \cdot
    \sup\limits_{\theta \in H} 
    \norm{\norm{
    \nabla \log p_{\theta}(X)
    }_{l^q}}_{L^q(P_\theta)}
    = C_q'
\end{align*}
where $p, q$ are conjugates.
Hence,
\begin{align*}
    C_q
    &=
    \sup\limits_{v\in H-\theta_0}
    \int_0^1 \norm{s_v(h, X)}_{L^q(P_{\theta_0+hv})} dh
    \\&\leq
    \sup\limits_{v\in H-\theta_0}
    \sup\limits_{h \in [0,1]}
    \norm{s_v(h, X)}_{L^q(P_{\theta_0+hv})}
    \\&\leq
    C_q'
\end{align*}
Since the resulting $\hat{U}(\theta)$ is no smaller after replacing $C_q$ with $C_q'$, the same conclusions in
Theorem~\ref{thm:main-o-net} must hold.
This concludes the proof. 

\end{proof}

\begin{corollary}[\bf Binomial Outcomes]\label{cor:binom-o-net}  
Consider the setting of Corollary~\ref{cor:main-o-net}.
Suppose further that $X \in \set{0,1}^{N\times d}$ 
are independent Bernoulli outcomes
with natural parameter $\theta \in \R^d$ such that
$T_i(X)$ is distributed $\Binom(N, p(\theta_i))$
for every $i=1, \ldots, d$ where $p$ is the sigmoid function.
Then, we may further upper bound $C_q'$
in Corollary~\ref{cor:main-o-net} with the following $C_q''$:
\begin{align*}
    C_q'' := \sup\limits_{v\in H-\theta_0} \norm{v}_{l^p}
    \cdot
    \br{
    \sum\limits_{i=1}^d
    \sup\limits_{\theta_i \in \pi_i(H)}
    \EEE_{\theta_i}\br{\abs{T_i-Np(\theta_i)}^q}
    }^{\frac{1}{q}}
\end{align*}
where $\pi_i(H) \subseteq \R$ 
is the projection of the tile, $H$, onto the ith standard basis,
and achieve the same conclusion as in Theorem~\ref{thm:main-o-net}.
\end{corollary}
\begin{proof}
From Corollary~\ref{cor:main-o-net},
\begin{align*}
    \norm{\norm{
    \nabla \log p_{\theta}(X)
    }_{l^q}}_{L^q(P_\theta)}
    &=
    \norm{\norm{
    T(X)-\nabla A(\theta)
    }_{l^q}}_{L^q(P_\theta)}
    \\&=
    \EEE_\theta\br{
    \sum\limits_{i=1}^d
    \abs{T_i(X) - \partial_i A(\theta)}^q
    }^{\frac{1}{q}}
    \\&=
    \br{
    \sum\limits_{i=1}^d
    \EEE_{\theta_i}\br{
    \abs{T_i(X) - \partial_i A(\theta)}^q
    }
    }^{\frac{1}{q}}
\end{align*}
Hence,
\begin{align*}
    \sup\limits_{\theta \in H}
    \norm{\norm{
    \nabla \log p_{\theta}(X)
    }_{l^q}}_{L^q(P_\theta)}
    &\leq
    \br{
    \sum\limits_{i=1}^d
    \sup\limits_{\theta \in H}
    \EEE_{\theta}\br{\abs{T_i(X)-\partial_i A(\theta)}^q}
    }^{\frac{1}{q}}
    \\&=
    \br{
    \sum\limits_{i=1}^d
    \sup\limits_{\theta_i \in \pi_i(H)}
    \EEE_{\theta_i}\br{\abs{T_i-Np(\theta_i)}^q}
    }^{\frac{1}{q}}
\end{align*}
where $\pi_i(H) \subseteq \R$ 
is the projection of the tile, $H$, onto the ith standard basis.

\end{proof}

\begin{remark}
Corollary~\ref{cor:binom-o-net} simplifies the software implementation because we can compute suprema over each dimension separately.
\end{remark}

The next theorem is an experimental one.
It is inspired by the techniques used in
Theorem~\ref{thm:main-o-net}.

\begin{theorem}\label{thm:holder-with-second}
Consider the setting of Theorem~\ref{thm:main-o-net}.
Define $\ell_\theta(x) = \log p_{\theta}(x)$.
Suppose further that for every $v \in H-\theta_0$
and $h \in [0, 1]$,
\begin{align*}
    \frac{\partial^2}{\partial h^2}
    \ell_{\theta_0 + hv}(x)
    \equiv
    \frac{\partial^2}{\partial h^2}
    \ell_{\theta_0 + hv}
\end{align*}
that is, the second derivative of $\ell_\theta$ does not depend on $x$,
and $\theta \mapsto \ell_\theta(x)$ is twice-continuously differentiable.
Define
\begin{align*}
    S(v, x)
    :=
    -\ell_{\theta_0 + v}(x) + \ell_{\theta_0}(x) 
    + \nabla\ell_{\theta_0}(x)^\top v
\end{align*}
Then, $S(v, x)$ does not depend on $x$, and
\begin{align*}
    f(\theta_0 + v)
    &\geq
    f(\theta_0)
    \exp\br{
    \frac{\nabla f(\theta_0)^\top v}{f(\theta_0)}
    - S(v)
    }
\end{align*}
where $S(v) := S(v, x)$.
\end{theorem}

\begin{proof}
Fix any $v \in H-\theta_0$.
Define the following:
\begin{align*}
    g(h) &:= f(\theta_0 + hv) \\
    s_v(h, x) &:= \frac{\partial}{\partial h} \ell_{\theta_0 + hv}(x)
\end{align*}
Then,
\begin{align*}
    \abs{g'(h)}
    &=
    \abs{\nabla f(\theta_0 + hv)^\top v}
    =
    \abs{\EEE_{\theta_0 + hv}\br{
    F(X) s_v(h, X)
    }}
    \\&\leq
    \EEE_{\theta_0 + hv}\br{
    \abs{F(X) s_v(h, X)}
    }
    \\&\leq
    \norm{F(X)}_{L^2(P_{\theta_0+hv})}
    \norm{F(X) s_v(h, X)}_{L^2(P_{\theta_0+hv})}
    \\&\leq
    \sqrt{g(h)} 
    \norm{F(X) s_v(h, X)}_{L^2(P_{\theta_0+hv})}
\end{align*}
Note that
\begin{align*}
    g''(h)
    &=
    \int F(x) \frac{\partial}{\partial h} 
    \br{s_v(h, x) \cdot p_{\theta_0+hv}(x)} d\mu(x)
    \\&=
    \EEE_{\theta_0+hv}\br{F(X) 
    \frac{\partial}{\partial h} s_v(h, X)
    }
    +
    \EEE_{\theta_0+hv}\br{F(X) s_v(h, X)^2}
    \\&=
    g(h) u_v(h) 
    +
    \EEE_{\theta_0+hv}\br{F(X) s_v(h, X)^2}
\end{align*}
where
\[
u_v(h) :=
\frac{\partial}{\partial h} s_v(h, x)
\]
Hence,
\begin{align*}
    \norm{F(X) s_v(h, X)}_{L^2(P_{\theta_0+hv})}
    &=
    \sqrt{g''(h) - g(h) u_v(h)}
\end{align*}
So, by substitution, noting that $g(h) \in (0,1)$
for the same reason as in Theorem~\ref{thm:main-o-net},
\begin{align*}
    \abs{g'(h)}
    &\leq
    \sqrt{g(h)\pr{g''(h) - g(h) u_v(h)}}
    \\ \implies
    g'(h)^2
    &\leq
    g(h) \pr{g''(h) - g(h) u_v(h)}
    \\ \implies
    \frac{g'(h)^2 - g(h) g''(h)}{g(h)^2}
    &\leq
    -u_v(h)
    \\ \implies
    \pr{\frac{g'(h)}{g(h)}}'
    &\geq
    u_v(h)
\end{align*}
Letting $f_1(h) := \frac{d}{dh} \log g(h)$,
by substitution and integration,
\begin{align*}
    f_1(h)
    &\geq
    f_1(0) + \int_0^h u_v(t) dt
    \\ \implies
    \log g(h)
    &\geq
    \log g(0) + f_1(0) h + \int_0^h \int_0^x u_v(t) dtdx
    \\ \implies
    g(h)
    &\geq
    g(0) \exp\br{f_1(0)h + \int_0^h \int_0^x u_v(t) dtdx}
    \\ \implies
    f(\theta_0+v)
    &\geq
    f(\theta_0)
    \exp\br{
    f_1(0) + \int_0^1 \int_0^x u_v(t) dtdx
    }
\end{align*}

Next, by Fubini's Theorem,
\begin{align}
    \int_0^1 \int_0^y u_v(t) dtdy
    &=
    \int_0^1 \int_0^1 u_v(t) \indic{t \leq y} dtdy
    =
    \int_0^1 u_v(t) \int_0^1 \indic{t \leq y} dy dt
    \nonumber
    \\&=
    \int_0^1 u_v(t) (1-t) dt
    =
    \int_0^1 \frac{d^2}{dt^2} \ell_{\theta_0+tv} \cdot (1-t) dt
    \label{eq:holder-with-second:no-x-dep}
    \\&=
    \int_0^1 \frac{d^2}{dt^2} \ell_{\theta_0+tv}(x) \cdot (1-t) dt
    \nonumber
    \\&=
    \ell_{\theta_0 + v}(x) - \ell_{\theta_0}(x) 
    - \nabla\ell_{\theta_0}(x)^\top v
    =
    -S(v, x)
    \nonumber
\end{align}
for any $x$.
The last line follows from Taylor's Remainder Theorem.
Note that $S(v, x)$ does not depend on $x$
since (\ref{eq:holder-with-second:no-x-dep}) does not.
Letting $S(v) := S(v,x)$, this gives us the simplified form:
\begin{align}
    f(\theta_0+v)
    &\geq
    f(\theta_0)
    \exp\br{
    f_1(0) - S(v)
    }
    \label{eq:holder-with-second:last-sub}
\end{align}

Finally, expanding out $f_1(0)$, we get that
\begin{align*}
    f_1(0)
    &=
    \frac{g'(0)}{g(0)}
    =
    \frac{\nabla f(\theta_0)^\top v}{f(\theta_0)}
\end{align*}
Substituting the above into (\ref{eq:holder-with-second:last-sub}), 
we arrive at the desired claim.

\end{proof}

\begin{remark}\label{rem:holder-with-second:exp-fam}
Exponential families satisfy the assumptions
of Theorem~\ref{thm:holder-with-second}.
Moreover, there is an explicit form for $S(v)$.
Specifically,
\begin{align*}
    S(v)
    =
    A(\theta_0+v) - A(\theta_0)
    - \nabla A(\theta_0)^\top v
\end{align*}
\end{remark}

\begin{corollary}\label{cor:holder-with-second:tie}
Under the setting of Theorem~\ref{thm:holder-with-second},
we have that
\begin{align*}
    f(\theta_0+v)
    &\leq
    1-(1-f(\theta_0))
    \exp\br{
    -\frac{\nabla f(\theta_0)^\top v}{1-f(\theta_0)}
    - S(v)
    }
\end{align*}
\end{corollary}

\begin{proof}
Let 
\begin{align*}
    \tilde{f}(\theta) 
    &:= 
    1-f(\theta) 
    = 
    \EEE_\theta\br{1-F(X)}
    =
    \EEE_\theta\br{\tilde{F}(X)}
\end{align*}
where $\tilde{F}(x) := 1-F(x)$.
By applying Theorem~\ref{thm:holder-with-second}
with $\tilde{F} \in [0,1]$,
\begin{align*}
    \tilde{f}(\theta_0+v)
    &\geq
    \tilde{f}(\theta_0)
    \exp\br{
    \frac{\nabla \tilde{f}(\theta_0)^\top v}{\tilde{f}(\theta_0)}
    - S(v)
    }
\end{align*}
Rearranging, we have our claim.
\end{proof}

\begin{corollary}
Assume the setting of Theorem~\ref{thm:holder-with-second}.
Further assume that $P_\theta$ has 
a log-concave density for every $\theta \in H$.
Define $v_m := \theta_m - \theta_0$ 
for $m=1,\ldots, M$, where $\theta_m$ are the 
vertices of the tile $H$.
Then,
\begin{align*}
    \sup\limits_{\theta \in H}
    f(\theta)
    &\leq
    1 - (1-f(\theta_0))
    \exp\br{
    -\max\limits_{m=1}^M \br{
    \frac{\nabla f(\theta_0)^\top v_m}{1-f(\theta_0)} + S(v_m)
    }
    }
\end{align*}
\end{corollary}

\begin{proof}
The proof is immediate from the fact that
\[
   v \mapsto \frac{\nabla f(\theta_0)^\top v}{1-f(\theta_0)} + S(v)
\]
is convex.
\end{proof}

%%% REMOVE FOR NOW %%%
\if 0
\subsection{The Parameter Space, Gridding, and Null Hypothesis Tests of Interest}

The parameter space in this three-armed Bernoulli example is given by $$(p_0,p_1, p_2) \in [0,1]^{3}.$$

In subsequent sections X through Y, we will work with a transformed set of parameters $\theta_i = log (p_i) - log(1 - p_i)$. This transformation is the canonical exponential family parametrization of the binomial distribution. We now have

$$(\theta_0, \theta_1, \theta_2) \in R^3$$

Note that the endpoints of the intervals, $p_i = 0$ and $p_i = 1$, have been lost. 
%Optional: we can discuss the topic of combinatorially dealing with these boundaries in subsection X
In this paper we shall not try to rescue them; rather, to ensure boundedness of the computation, we shall focus on a compact set 

$$\{ (\theta_0, \theta_1, \theta_2) \in \Theta_0 \subset R^3 \}$$

In our example, we approach this by simply expanding a grid of values for each $p_i$:

$$p_i \in (.2, .28, ... , .8)$$

which results in the grid given by

%$$\theta_i \in ( logit(.2), logit(.28), \ldots , logit(.8)) =
$$
\theta_i \in (-1.386, -.944, \ldots , (1.386) )$$

We can make a list of all 3-tuples composed of these sequences in positions $1$ thru $G$ (where $G$ is the length of the grid) and then index this list by $j$ in 1...J. Thus $J = length(seq(.2, .8, by = .1))^3$. Then, we may write our grid-points as: %(\textit{disambiguate! by bolding or something like this for the vectors of theta})

$$\theta_j =(\theta_{j_1},\theta_{j_2},\theta_{j_3})$$.

To each $\theta_j$ we will associate a volume $H_j$ so that their union covers $\Theta_0$. We define the boundaries of each $H_j$ as follows:

$$ \{ \theta : a \leq \theta \leq b\} \cap \Theta_0$$

where the vector inequalities $\leq$ apply to every index. Thus, each $H_j$ is either a hyper-rectangle, or a hyper-rectangle with its portion outside of $\Theta_0$ removed.
For hypothesis testing and inference, we may be interested in the quantities $p_i$ individually; or the differences $p_i - p_j$ for $i \neq j$; or the selected treatment arm $p_*$; or its comparison against control $p_* - p_0$. For our example, here is a list of relevant null hypotheses we could consider:

\begin{itemize}
    \item $H_1: p_1 \leq c$
    \item $H_2: p_1 \leq p_0$ 
    \item $H_3: p_* \leq c$
    \item $H_4: p_* \leq p_0$
\end{itemize}

Our methods can offer bounds on the rejection probabilities of hypothesis tests for each of these quantities in Section X; can tune tests, so that the overall procedure can maintain a uniform Type I Error bound; can give confidence Intervals, as described in Section W; and can bound the bias and variance of bounded estimators, as described in Section Z.

\subsection{The Likelihood Model}

In this example, the likelihood is determined by the sufficient statistics: $x_{02}$, the total sum of successes in the control group; $x_{11}$ and $x_{21}$, sums of successes at the first interim from $A_1$ and $A_2$ respectively; and $x_{12}$ or $x_{22}$, their sums of successes from the second stage, depending on which treatment arm is selected to continue. The likelihood is thus:

$$\mathbbm{1}\{x_{11} < x_{21} \} {50 \choose x_{11}} p_1^{x_{11}} (1 - p_1)^{50 - x_{11}}{250 \choose x_{22}}p_2^{x_{22}} (1 - p_2)^{250 - x_{22}}{250 \choose x_{02}}p_0^{x_{02}} (1 - p_2)^{250 - x_{02}} + $$

$$\mathbbm{1}\{x_{11} \geq x_{21} \} {250 \choose x_{12}} p_1^{x_{12}} (1 - p_1)^{250 - x_{12}}{50 \choose x_{21}}p_2^{x_{21}} (1 - p_2)^{50 - x_{21}}{250 \choose x_{02}}p_0^{x_{02}} (1 - p_2)^{250 - x_{02}} $$

We may reparametrize with the exponential family parameters, $$\theta_i = log(p_i / (1 - p_i)).$$

The result is

$$\mathbbm{1}\{x_{11} < x_{21} \} {50 \choose x_{11}}{250 \choose x_{22}}{250 \choose x_{02}}
e^{x_{11} \theta_1 + x_{22} \theta_2 + x_{02} \theta_0 - 50 \log(1 + e^{\theta_1})  - 250 \log(1 + e^{\theta_2}) - 250 \log(1 + e^{\theta_0})} + $$

$$\mathbbm{1}\{x_{11} \geq x_{21} \} {250 \choose x_{12}}{50 \choose x_{21}}{250 \choose x_{02}}
e^{x_{12} \theta_1 + x_{21} \theta_2 + x_{02} \theta_0 - 250 \log(1 + e^{\theta_1})  - 50 \log(1 + e^{\theta_2}) - 250 \log(1 + e^{\theta_0})}.$$

If we denote the final sample sizes $n = (n_0, n_1, n_2)$, we may define the vector $\mu := (n_0 p_0, n_1 p_1, n_2 p_2)$ and the matrix $\Sigma := diag( n_0 p_0 (1 - p_0), n_1 p_1 (1 - p_2), n_2 p_2 (1 - p_2))$, and write the observed sums of successes $y = (y_0, y_1, y_2)$. Then we will notice that the gradient and Hessian of this likelihood with respect to $\theta$ obey

$$\nabla L = (y - \mu) L.$$

$$\nabla^2 L = ((y - \mu)(y - \mu)^T - \Sigma ) L$$.

Based on Sections X of [Sklar 2021], we have the following results for this model:

Assume we have a Monte Carlo simulation of the trial given a fixed parameter vector $\theta$, which yields i.i.d. draws of the trial results $(y_i, n_i)$ for $i$ in $1, \ldots, I$. Then, for any set $S$ which is determined by the trial's outcomes $X$,

\begin{enumerate}
\item $E[ (y_i - \mu_i) \mathbbm{1}\{(y_i,n_i) \in S\} ] = \nabla Pr_{\theta}\{S\}$

\item $Cov[ (y_i - \mu_i) \mathbbm{1}\{(y_i,n_i) \in S\}] \preccurlyeq \Sigma_{max} $

where $A \preccurlyeq B$ means that $B - A$ is positive semidefinite, and $$\Sigma_{max} := diag( 250 p_0 (1 - p_0), 250 p_1 (1 - p_2), 250 p_2 (1 - p_2)).$$

\item $\frac{1}{I} \sum \limits_{i=1}^{I} v^T (y_i - \mu_i) \mathbbm{1}\{(y_i,n_i) \in S\} + \sqrt{\frac{v^T \Sigma_{max} v}{I} (\frac{1}{\delta} - 1) }$

is a $1 - \delta$ confidence interval for $\nabla Pr_{\theta}\{S\}$.

\item $\sum \limits_{i=1}^{I} \mathbbm{1}\{(y_i,n_i) \in S\}$ has distribution $Binomial(n = I, p = Pr_{\theta}\{S\})$. For a confidence interval on $Pr_{\theta}\{S\})$, one may invert Theorem 1 of \cite{short2013improved}, which states that for a binomial, for $k$ between $1$ and $n - 2$

$$\Phi( sign (k - np) \sqrt{2 n D(p, k/n)} )$$

$$ \leq P(X \leq k)$$

$$ \leq \Phi( sign (k + 1 - np) \sqrt{2 n D(p, (k + 1)/n)} )$$

where

$D(p,c) = c ln(c/p) + (1 - c) ln((1-c)/(1-p))$

\item $\nabla^2 Pr_{\theta} \{S\} \preccurlyeq \Sigma_{max}$

\end{enumerate}

It is worth noting in the above statements that $\mu_i$ varies according both the parameter vector $\theta$ and simulation instance, and $\Sigma_{max}$ varies according to the parameter vector $\theta$.


\subsection{Bounds on Probabilities}

In this section we will show how to achieve bounds on Type I Error and power. We apply the methods described in Section X of [Sklar 2021] to the null hypothesis $H_4$ in Section Y, as well as to the power function. We will take $H_4: p* \leq p_0$ as our motivating example: comparing the selected arm against the control arm.
To control Type I Error of $H_4$, we shall split up our hypothesis rejections into two disjoint sets, based on the arm selected: $S_1$, which occurs if treatment arm $A_1$ is selected and declared successful and $p_1 \leq p_0$; and $S_2$, if treatment arm $A_2$ is selected and declared successful and $p_1 \leq p_0$. The upshot of this division is that on these sets, our parameters of interest are not random.

We may further simplify the issue by defining our grid-volumes $H_j$ such that $\mathbbm{1}\{p_i \leq p_0 \}$ will always remains constant over each $H_j$. [This may require either a re-parametrization of the grid-space, rotating it so that we parametrize in terms of $\theta_i$ - $\theta_0$; or, chopping our volumes in half along the boundary line]. Thus, our remaining problem is to control uniformly over each $H_j$ the probability that $A_i$ is selected and declared successful.

Following [Sklar 2021], our approach will be to take a second-order Taylor expansion of this probability, and bound all three terms separately. Without loss of generality, it suffices to consider to upper bounds, as a lower bound may be achieved by upper bounding $P(S_1^C)$. Taylor Expansion yields the following equality:

$$ Pr_{\theta}\{S_1\} = Pr_{\theta_j}\{S_1\} + (\theta - \theta_j) \nabla Pr_{(\cdot)}\{S_1\} (\theta_j) + \int \limits_{\alpha = 0}^1 (1 - \alpha) (\theta - \theta_j)^T \left[ \nabla^2 Pr_{(\cdot)}\{S_1\} (\theta + \alpha (\theta - \theta_j) ) \right] (\theta - \theta_j)$$

Let us visualize some pieces of this puzzle:

[figure 1] here are our unbiased estimates of $Pr_{\theta}{S_1}$ from Monte Carlo, evaluated at each $\theta_j$. (shown with coloring or 3D)

[figure 2] (shown as directional vectors sticking out from each point $\theta_j$), here are our unbiased estimates of $\nabla Pr_{\theta_j}\{S_1\}$, according to equation X (in previous section).

Note that we also have

$$ Pr_{\theta}\{S_2\} = Pr_{\theta_j}\{S_2\} + (\theta - \theta_j) \nabla Pr_{(\cdot)}\{S_2\} (\theta_j) + \int \limits_{\alpha = 0}^1 (1 - \alpha) (\theta - \theta_j)^T \left[ \nabla^2 Pr_{(\cdot)}\{S_2\} (\theta + \alpha (\theta - \theta_j) ) \right] (\theta - \theta_j)$$

We may unite these equations in this case (the story will be slightly more difficult in Section X, for bias), yielding (if we define $S := S_1 \cup S_2$)

$$ Pr_{\theta}\{S\} = Pr_{\theta_j}\{S\} + (\theta - \theta_j) \nabla Pr_{(\cdot)}\{S\} (\theta_j) + \int \limits_{\alpha = 0}^1 (1 - \alpha) (\theta - \theta_j)^T \left[ \nabla^2 Pr_{(\cdot)}\{S\} (\theta + \alpha (\theta - \theta_j) ) \right] (\theta - \theta_j)$$

Ultimately, we wish to upper bound this over $\theta \in H_j$ for each (disjoint) $H_j$. So we may write conservatively:

$$\sup \limits_{\theta \in H_j} Pr_{\theta}\{S_1\} \leq Pr_{\theta_j}\{S_1\} + \sup \limits_{\theta \in H_j} (\theta - \theta_j) \nabla Pr_{(\cdot)}\{S_1\} (\theta_j) + \sup \limits_{\theta, \theta' \in H_j} \frac{1}{2} (\theta - \theta_j)^T \left[ \nabla^2 Pr_{(\cdot)}\{S_1\} (\theta') \right] (\theta - \theta_j)$$





We will estimate the first two terms via Monte Carlo and upper bound them with  confidence intervals. The third term can be upper bounded directly. Key parts of these bounds, originally from [Sklar 2021], are given in the previous section X.
Enumeration point 4 allows us to construct an upper confidence bound on $Pr_{\theta}\{S\}$ with a predetermined confidence level 1 - $\delta_{j,1}$, using binomial probabilities or an approximation.
Equation point 3 allows us to construct an upper confidence bound on $v^T \nabla Pr_{(\cdot)}\{S\}(\theta_j)$ with a predetermined confidence level 1 - $\delta_{j,2}$; and as described in [Sklar 2021], for a convex $H_j$ it suffices to evaluate this upper bound for $v = (\theta - \theta_j)$ corresponding to taking $\theta$ on each of $H_j$'s corners, and then take the maximum of the resulting confidence bounds. Finally, we can directly upper bound the third term since 

$$ \nabla^2 Pr_{(\cdot)}\{S\}(\theta') \preccurlyeq diag( 250 \sup \limits_{p_0 \in H_j} {p_0 (1 - p_0)}, 250 \sup \limits_{p_1 \in H_j} {p_1 (1 - p_1)} , 250 \sup \limits_{p_2 \in H_j} {p_2 (1 - p_2)}    )$$

Substituting this for the Hessian in the third term on the right side of equation X, if $H_j$ is convex it suffices to check values of $\theta$ at the corners $\theta_1, \ldots, \theta_m$ of $H_j$ and return as our upper bound the greatest value achieved by

$$\frac{1}{2} (\theta_m - \theta_j)^T  \left[ diag( 250 \sup \limits_{p_0 \in H_j} {p_0 (1 - p_0)}, 250 \sup \limits_{p_1 \in H_j} {p_1 (1 - p_1)} , 250 \sup \limits_{p_2 \in H_j} {p_2 (1 - p_2)}    ) \right] (\theta_m - \theta_j).$$


%Here we describe in detail the process for establishing a Type I Error upper bound for each individual $p_i$.

%[at the end, can discuss: reparametrization]

%More Detailed [perhaps in the appendix?]

%Key characteristics of the trial design such as power, Type I Error, and can be expressed as probabilities of events, and written as

%$$E[1_{F}]$$ for some event $F(\theta,X)$.

The result is an upper bound to the Type I Error probability which is valid over $H_j$ with confidence $1 - \delta_{j,1} - \delta_{j,2}.$

Here we display the error introduced by the approximation of the first term:

[figure]

second term:

[figure]

third term:

[figure]

(these may go into the appendix.)

\fi
%%% END REMOVE %%%

%%% BEGIN REMOVE %%%
\if 0
\section{Appendix C: Tuning the Critical Value}

[Note: this is duplicated from the discussion section. Which should we cut, if either?] In this appendix section, we study how Type I Error can be tuned to be kept under a fixed level (such as 2.5\%), discussing 3 different approaches. The features of these approaches are summarized in the following table \footnote{The ``Bias" row refers to the tuning bias per representative point (and its surrounding space). But, the typical approach for tuning a design is to take the most conservative tuning to establish control over ALL subregions. This approach will typically leads to additional conservativeness, except in cases where the worst-case-Type-I-Error point is so prominent that tuning is almost certain to hinge on that single region}:

\begin{center}
\begin{tabular}{|c|c|c|c|} 
 \hline
 Approach & 1. Confidence & 2. Naive & 3. Poissonized \\ [0.5ex] 
 \hline\hline
 Rigorous Control & Yes & Special Cases & Yes \\ 
 \hline
 Intuitiveness & Medium & High & Low \\
 \hline
 Bias & $\tilde{O}(1/\sqrt{n})$ & $\tilde{O}(1/n)$ & $\tilde{O}(1/n)$ \\
 \hline
\end{tabular}
\end{center}

Approach 1 is the rigorous and conservative confidence-bound based tuning discussed earlier in Section X, first given in \cite{sklar:2022}. %we use the confidence bounding approach in Sections X to construct a $2.5\% - \delta$ interval, and show that the probability that we choose a rule more conservative than $2.5\% - \delta$ is less than $\delta$, achieving an overall guarantee.
Approach 2 is an intuitive and ``naive" approach, where the empirical estimate of Type I Error is tuned without paying for upper confidence bounds, stopping when the estimated Type I Error crosses 2.5\% . We characterize its performance and argue that its Type I Error is well-behaved in almost all reasonable cases. However, due to the possibility of overshoot, rigorous Type I Error control only holds in special cases. Approach 3 does rigorously control the Type I Error and is asymptotically less conservative than Approach 1, but it is slightly more complicated than the other two approaches and requires more simulations than Approach 2 by a factor of roughly $\frac{2}{1-\alpha}$ to achieve similar performance. The key mathematical principle underlying Approach 3 is to control Type I Error by constructing a martingale for the empirical estimate of the first two Taylor terms of the Type I Error. As part of this construction, it is required to perform a Poisson number of simulations. Overshoot is dealt with by taking a second set of simulations and ``reversing" the process until the estimate crosses back below 2.5\%. In future work this approach may be amenable to potential extensions, such as tuning or optimizing the design in multiple dimensions, or using importance sampling to reduce the number of necessary simulations.

%In Section~\ref{ssec:type-I-error}, 
%we demonstrated how it is possible to give an upper 
%(and thus, correspondingly a lower) confidence bound 
%on the Type I Error function. 
%There is a notable shortcoming to using this approach directly 
%for a regulatory process: the quality of the upper bound 
%is subject to the randomness of the simulation, 
%so that an $\alpha$ level guarantee is not necessarily assured. 

\subsection{Tuning Approach 1: Confidence-Based}

Sklar (2021) first described this procedure for tuning a design's 
rejection thresholds to ensure that an overall $\alpha$ level guarantee 
can be achieved tightly and conservatively \cite{sklar:2022}. This approach embeds the design in a 
\emph{monotone family} of rejection rules with a 1-dimensional tuning parameter $\lambda$, 
such that increasing $\lambda$ strictly increases the rejection set. 
As an example, if a design uses the z-statistic to make upper-tail rejections with critical value $z^*$, it is natural to index this family via the tuning parameter $\lambda := -z^*$. Equivalently, we could use the p-value threshold for the naive z-test, because each critical z-thresholds maps monotonically to a p-value threshold. 

Then, we must search for the optimal value of $\lambda$ such that our Type I Error upper bound from Section~\ref{ssec:type-I-error} 
is tightly under our desired $\alpha$ level. We may stop just before the first choice of $\lambda$ where 2.5\% is exceeded.
We now present this result as a theorem.

\begin{theorem}\label{thm:tuning}
Consider the setup of Theorem~\ref{thm:main},
where we have instead a function $F_{\theta, \lambda}(x)$
that is twice-continuously differentiable with respect to
$\theta \in H$,
$f_{\lambda}(\theta) := \EEE_\theta\br{F_{\theta,\lambda}(X)}$
where $X \sim P_{\eta(\theta)}$,
and there exists $\hat{U}_{0}(\lambda)$,
$\hat{\Delta}_m(\lambda)$,
and $U_R(v,\lambda)$ that satisfy Assumptions~\ref{ass:main-0th}-\ref{ass:main-2nd},
respectively.
Define
\begin{align*}
    \hat{U}(\lambda)
    :=
    \hat{U}_0(\lambda)
    +
    \max\limits_{m=1}^M \br{\hat{\Delta}_m(\lambda) + U_R(v_m,\lambda)}
\end{align*}
similarly as in Theorem~\ref{thm:main}.
For any $\alpha \in [0,1]$, define
\begin{align*}
    \lambda^* &:= \inf\set{\lambda : f_{\lambda}(\theta) > \alpha} \\
    \alpha_+ &:= f_{\lambda^*-}(\theta) 
    := \lim\limits_{t \uparrow \lambda^*} f_t(\theta)\\
    \alpha_- &:= f_{\lambda^*+}(\theta)
    := \lim\limits_{t \downarrow \lambda^*}
    f_t(\theta)
\end{align*}
Let
\begin{align*}
    \hat{\lambda}^*
    :=
    \inf\set{\lambda : \forall \lambda'' > \lambda,\, \hat{U}(\lambda'') < \alpha_-}
\end{align*}
be finite a.s.
Assume further the following additional conditions:
\begin{enumerate}
    \item $\lambda^*$ is finite.
    
    \item For every $\theta \in H$,
    $\lambda \mapsto f_{\lambda}(\theta)$
    is monotonically decreasing and right-continuous at $\lambda^*$.
\end{enumerate}
Then, for any random $\hat{\lambda} > \hat{\lambda}^*$ a.s.
and any $\theta \in H$,
\begin{align}
    \prob\br{f_{\hat{\lambda}}(\theta) \leq \alpha_+}
    \geq
    1-\delta
    \label{eq:thm:tuning:main}
\end{align}
\end{theorem}

\begin{proof}
Fix any (random) $\hat{\lambda}$ such that $\hat{\lambda} > \hat{\lambda}^*$
and $\theta \in H$.
Note that by right-continuity, $f_{\lambda^*}(\theta) = \alpha_-$.
Note also that if $\hat{\lambda} > \hat{\lambda}^*$ a.s.,
then $\hat{U}(\hat{\lambda}) < \alpha_-$ a.s.
by definition of $\hat{\lambda}^*$.
We then have that
\begin{align*}
    \prob\br{f_{\hat{\lambda}}(\theta) > \alpha_+}
    &\leq
    \prob\br{f_{\hat{\lambda}^*}(\theta) > \alpha_+}
    \leq
    \prob\br{\lambda^* > \hat{\lambda}^*}
    \leq
    \prob\br{\hat{U}(\lambda^*) < \alpha_-}
    \\&\leq
    \prob\br{\hat{U}(\lambda^*) < f_{\lambda^*}(\theta)}
    \leq
    \delta
\end{align*}
\end{proof}

\begin{corollary}\label{cor:thm:tuning}
Under the setting of Theorem~\ref{thm:tuning},
if $F_{\theta, \lambda}(x)$ is the indicator defined in Section~\ref{ssec:type-I-error}
where the rejection set shrinks as $\lambda$ increases,
and $f_{\lambda}(\theta)$ is continuous,
then the result of Theorem~\ref{thm:tuning} holds.
\end{corollary}

\begin{proof}
The proof is immediate since $\lambda \mapsto f_{\lambda}(\theta)$
is monotonically decreasing if the rejection set shrinks as $\lambda$ increases.
\end{proof}

\begin{remark}
In Theorem~\ref{thm:main}, it is not immediate to get a guarantee as in (\ref{eq:thm:tuning:main}) for a fixed $\lambda$.
It is precisely because we do not have the guarantee that
$\lambda > \hat{\lambda}^*$ (a.s.) for a fixed $\lambda$.
The purpose of Theorem~\ref{thm:tuning} is to tune the $\lambda$
by randomly selecting it to achieve this guarantee.
\end{remark}

\begin{remark}
In Corollary~\ref{cor:thm:tuning}, if the true Type I Error function
is discontinuous, one can change $F_{\theta, \lambda}(x)$ such that
the test is randomized so that $\lambda \mapsto f_{\lambda}(\theta)$
achieves $\alpha$.
\end{remark}

\begin{remark}
In Corollary~\ref{cor:thm:tuning}, 
one can choose $\hat{U}_0(\lambda)$, $\hat{\Delta}_m(\lambda)$, $U_R(v,\lambda)$
as described in Section~\ref{ssec:type-I-error}.
\end{remark}

\begin{remark}
Similar to Corollary~\ref{cor:main},
we may extend the result of Theorem~\ref{thm:tuning}
to the case of a platten by repeatedly
applying Theorem~\ref{thm:tuning}.
\end{remark}

\begin{subsection}{Approach 2: Naive Empirical Tuning}


\section{Analysis of Naive Simulation Tuning}

(put this earlier)

Given our simulation set, we may define $\hat{\alpha}(\lambda) := FILL_IN!$

One may raise the following natural question: what would happen if tuned our procedure, stopping at the value of $\lambda$ where this empirical estimate exceeds 2.5\% ? We define

$$ \lambda^* := \inf \{\lambda : \sum \hat{\alpha}(\lambda) > .025 \}$$

In this case, there are two natural questions to ask:

(1) Is $E[\hat{\alpha}(\lambda^*)]$ biased for $E[\alpha(\lambda^*)]$?

(2) How large is the overshoot of $\hat{\alpha}$ past 2.5\%, and can we bound it easily?

It turns out that in general, the answer to (1) is ``yes"; and under 'typical' conditions, one should expect a conservative bias, in the sense that in expectation, $\hat{\alpha}(\lambda^*)$ is larger than $\alpha(\lambda^*)$. We derive a formula for this quantity in the following subsection, and in usual cases it will be seen to be positive.

(2) since there are $n$ simulations this overshoot one should typically expect this should be bounded on order $O(1/n)$; but perhaps surprisingly, an adversary could design a pathological case so that this is not true with any fixed constant. We describe the construction of such a pathological case in subsection X. Such cases are not expected to be of any reasonable concern for clinical trial design; but in appreciation the value of an unqualified proof, in Section X we are motivated to present a completely alternative approach with an airtight proof statement, at the cost of requiring a greater number of simulations.

\subsection{Analysis of the bias under naive tuning, via the Hot Deck Lemma}

In black jack, if one has seen few aces and high cards, there are more of them remaining in the deck, and the deck is said to be ``hot." This fact is fundamental to why blackjack is a beatable game, if one continues to play and bets larger when the deck is hot.

In our tuning scenario, if one has not yet observed $\hat{\alpha}(\lambda) > 2.5\%$ then there are probably more p-values above $\lambda$ and they will subsequently arrive with greater intensity, causing $\hat{\alpha}(\lambda^*)$ to be conservatively biased. We may mathematize this as follows:

Define the filtration 

$$ F_t := \sigma \left( p_i, h_i : p_i \leq \lambda \right)$$

Define $N_t$ as the number of ``live" p-values, $N_t := \sum \limits_i \mathbbm{1} \{p_i  > t\}$

Define $\alpha(t) := E[h_i \mathbbm{1} \{p_i  \leq t\}]$

Then, I claim:

$$M(s) := \hat{\alpha}(s) - \int \limits_{0}^s \alpha'(t) \frac{N_t}{N(1-t)}$$

(Why? This is actually slightly nontrivial I think. This could come from pasting together a bunch of stopping times, and showing that at each step, the stopped quantity is still a martingale, using an argument with epsilons and deltas to show that we can isolate the stopping times from each other.)

We may then write:

$$M(s) := \hat{\alpha}(s) - \alpha(s) + \int \limits_{0}^s \alpha'(t) \left[1 - \frac{N_t}{N(1-t)}\right]$$

Then by optional stopping, for any stopping time $\tau$,

$$0 = M(0) = E[M(\tau)] = E[\hat{\alpha}(\tau) - \alpha(\tau)] 
+ E\left[ \int \limits_0^1 \mathbbm{1} \{p_i \leq \tau \} \alpha'(t) \left[1 - \frac{N_t}{N(1-t)}\right] \right]$$
 
Thus, $\hat{\alpha}(\tau)$ is a conservative estimator if and only if

$$E\left[ \int \limits_0^1 \mathbbm{1} \{p_i \leq \tau \} \alpha'(t) \left[1 - \frac{N_t}{N(1-t)}\right] \right] \geq 0$$

Notice that if $\tau'$ were independent of $N_t$ this integral would collapse to zero.

Thus we may subtract such an integral for an independent copy $\tau'$, to rewrite this as

$$= E\left[ \int \limits_0^1  \frac{\alpha'(t) }{N}(1-t) \left[ P(t \leq \tau') N_t - \mathbbm{1}\{t \leq \tau\} N_t \right] dt \right]  \geq 0$$

Splitting $N_t$ into a sum of $N$ i.i.d. indicators, we can cancel the factor of $N$

$$=- E\left[ \int \limits_0^1  \frac{\alpha'(t) }{1-t} \left[ P(t \leq \tau') t - P(t \leq \tau, p_t \leq t) \right] dt \right]  \geq 0$$

(can this simplify further by re-arranging t to cancel with 1-t? I think so, try this!)

In almost all reasonable cases, it should be the case that knowing $p_t<s$ increases the chance that $\tau$ has been hit by time $s$, and thus the integrand is positive.

This is true if $h_i>0$.

In general case, for almost all problems one could safely hand-wave this as being morally true, in that it fail for some pathological or adversarially constructed cases.


\end{subsection}

\begin{subsection}{Approach 3: An alternative tuning approach with a Poissonized Martingale}

This section provides an alternative method for tuning with full Type I Error control\footnote{This proof holds in expectation for the average design. Fortunately, the expected Type I Error IS the procedure Type I Error}, which may be less conservative than the procedure described in Section X. This alternative approach tunes directly on an unbiased Type I Error estimate, omitting the confidence widths on the 0th and 1st order terms of our Taylor expansion. We study a naive version which stops at the first value of $\lambda$ where the empirical estimate of Type I Error breaks 2.5\%, in Section Y. To ensure a guarantee and prevent overshoot, in Section Z we modify that procedure in several ways. Rather than a fixed number of say 10,000 simulations per grid-point, we would perform a Poisson (10,000) number of simulations \footnote{One hopes that one will not get an arbitrarily unlucky amount of runtime; fortunately the Poisson is not a long-tailed distribution}. On net, compared to a naively tuned Type I Error estimate, our Type I Error guarantee is variance-inefficient by an asymptotic factor of about $2/(1 - 2.5\%)$; but in exchange for that price, we get a rigorous, provable guarantee, which the naive approach lacks.

Our approach is to create a martingale, so that our unbiased estimator of the Type I Error. To achieve this martingale structure, we must also use an estimator with a slightly different normalization. Plus, at the point where we jump over the 2.5\% threshold, we are likely to have some small extra spillover. If this is undesirable, one may run an entirely new set of simulations to tune our Type I Error estimate back down, so that we safely stop below 2.5\%. To account for the remote possibility that we fail to stop back below $2.5\%$, we inflate our guarantee slightly with a tail bound based on fourth moments.

We assert here that this Poissonization technique can be generalized to handle tuning across multiple dimensions or general sets in the fashion of ADAPT-STAR (cite Ramdas et al’s sequential-revealing ideas), though we leave such a full treatment to future work.

\subsection{Martingale Construction}

We shall draw:

$N_1 \sim Poisson(n), N_2 \sim Poisson(n)$.

We assume that our tuning family rejects according to some statistic, $s \leq t$, where WLOG we may have $t$ range from $0$ to $1$. Assume that $(s^j_i, h^j_i)$ are sequences of i.i.d. simulation draws of the rejection statistic and an associated weight function of interest, for $j = 1,2$ and $i=1, 2, \ldots$. (Typically we might have $h = 1 + v^T(T(X_i) - \nabla A(\theta))$. This choice is intended to yield the combined estimator of 0th and 1st order terms, for a specific direction vector $v$.) Without loss of generality, we may re-map our rejection statistics (via some monotone function not known to the analyst) into p-values $p_i$ such that $P(p_i < t) = t$.

Then, define

$$\hat{\alpha}^1(t) := \frac{1}{n} \sum \limits_{i=1}^{N^1} h_i^1 \mathbbm{1}_{p^1_i \leq t}$$

$$\alpha^1(t) := E[\hat{\alpha}^1(t)]$$

$$M^1_t := \hat{\alpha}^1(t) - \alpha^1(t)$$

$$F^1_t := \sigma \left( (p_i^1, h_i^1): p^1_i \leq t, i \leq N^1 \right)$$

Thus the sequence of $\{p_i^1 : i \leq t \}$ is a Poisson point process with intensity $n$. We could, alternatively, construct this process in a way which is clearly memoryless, using the exponential waiting times representation. Then, by the memoryless property, if $s > t$ for some times $s,t$,

$$E[ M_s^1 | F_t^1]
=M_t^1 + E[M^1_s - M^1_t | F^1_t]
=M_t^1 + E[M^1_s - M^1_t]
=M_t^1 + M^1_s - M^1_t = M_1^T$$

And thus the martingale property is verified.

We can define a stopping time for when we first hit or break an estimate of 2.5\%:

$$\tau^1 := \inf \{t: \hat{\alpha^1}(t) \geq 2.5 \% \}$$

If there is no such time and $\hat{\alpha^1}(1) < 2.5\%$, we may set $\tau^1 = 1$ and terminate our procedure at the least conservative possible setting, i.e.,``reject everything"

Otherwise, we have most likely overshot past 2.5\%, and we will wish to correct our overshoot. therefore we 
shall pause $M^1_t$ for the time being at $\tau^1$; and from that point forward paste onto it a new martingale. To construct the second pieces, define

$$\hat{\alpha^2}(t) := \frac{1}{n}\sum \limits_{i=1}^{N^2} h^2_i \mathbbm{1}\{ \tau^1 - (t - \tau^1) < p^2_i < \tau^1\}$$

$$\alpha^2(t):= E[\hat{\alpha^2}(\tau^1) - \hat{\alpha^2}( \tau^1 - (t - \tau^1)|\tau^2]$$

Note that if we look at $\alpha^1(t)$ for $t \leq \tau_1$ and $\alpha^1(\tau_1) - \alpha^2 (t)$ for $t > \tau_1$, it should look like a symmetric pyramid of sorts, with a center at $(x=\tau_1,y=\alpha^1(t))$, and a left leg at $(x=0,y=0)$.

Now let $M^2_t := \hat{\alpha^2}(t) - \alpha^2(t)$.

Observe similarly that for $t$ between $\tau_1$ and $2\tau_1$, $M^2_t$ is a martingale with respect to

$$F^1_t := \sigma \left( (p_i^2, h_i^2): \tau^1 - (t - \tau^1) < p^2_i < \tau^1, i \leq N^1 \right)$$

Then set

$$M_t := 
\mathbbm{1}\{t \leq \tau_1\}M_t^1 + \mathbbm{1}\{t > \tau_1\}[M_t^1 - M^2_t]$$

Define $\tau_2$ as the next stopping point $t > \tau_1$ where $\hat{\alpha(t)} = \hat{\alpha^1(\tau_1)} - \hat{\alpha^2(t)} \leq 2.5\%$. If $\tau_1=1$ stop immediately with $\tau_2 = \tau_1 = 1$ and let $\hat{\alpha^2} = \alpha^2(\tau) = 0$. If we overshot $2.5\%$ the first time but we cannot make it back under by time $2\tau_1$, stop at time $\tau_2 = 2\tau_1$. This is the only case in which $\hat{\alpha}(t) > 2.5\%.$

Now consider the rule that uses the tuning value $\lambda^* = 2\tau^1 - \tau^2$ where we stopped. Then by optional stopping,

$$0 = E[M_{\tau^2}] = E[M^1_{\tau^1} - M^2_{\tau^2}] = E[\hat{\alpha^1}(\tau^1) - \alpha^1(\tau^1) - \hat{\alpha^2}(\tau^2) + \alpha^2(\tau^2)] = E[\hat{\alpha}(\tau^2) - \alpha(\lambda^*)].$$

Where by construction, $\hat{\alpha}(\tau^2) \leq 2.5\%$ in all cases, except the case where $\tau^2 = 2 \tau_1$. Note also that when $\tau^2 = 2\tau^1$, $\alpha(\tau^2) = 0$. Hence,

$$E[\alpha(\lambda^*)] = E[\alpha(\tau^2) = E[\hat{\alpha}(\tau^2))]]$$
by optional sopping of the martingale

$$ \leq E[2.5\% \mathbbm{1}\{\tau^2 < 2\tau^1\}] + E[\hat{\alpha}(\tau^2) \mathbbm{1}\{\tau^2 = 2 \tau_1\}]$$

$$\leq 2.5\% + E[\left(\hat{\alpha}(\tau^2) - 2.5\% \right)\mathbbm1 \{\tau^2 = 2 \tau^1 \}]$$

Now we may bound

$$E[\left(\hat{\alpha}(\tau^2) - 2.5\% \right)\mathbbm1 \{\tau^2 = 2 \tau^1 \}] = 
E[\left(\hat{\alpha}(\tau^2) -\alpha(\tau^2) - 2.5\% \right)\mathbbm1 \{\tau^2 = 2 \tau^1 \}]
,$$

noting $\alpha(\tau^2)=0$ when $\tau^2 = 2\tau^1.$

$$\leq E[\left(\hat{\alpha}(\tau_2)-\alpha(\tau_2) - 2.5\% \right)^+]$$

$$ \leq \int \limits_{x=0}^\infty x P(\hat{\alpha}(\tau^2)- \alpha(\tau^2) - 2.5\% > x) dx$$

We now derive a tail bound, which will be used to bound the inside of this integral, after which we shall return and evaluate this loss.

\subsubsection{Tail bound}

We seek a bound on 

$E[\left(\hat{\alpha}(\tau^2) - \alpha(\tau^2) \right)^4]$ in order to get the tail bound for the inside of the integral.

Note that we could extend the martingale further beyond $\tau^2$ by ``running both martingales all the way forward" to include all data, by adding a final time $T$ where

$$F_T = \sigma( p_i^j,h_i^j | j \in \{1,2\}, i \leq N^j)$$

$$M_T = 
\frac{1}{n}\sum \limits_{k=1}^{N^1} h_k - 
\frac{1}{n}\sum \limits_{l=1}^{N^2}  h_l$$

Appending this to the end of $M_t$, we observe that $M_t$ is still a martingale. Then, because $g(u) = u^4$ is a convex function, $M_t^4$ is a sub-martingale. Therefore,

$$E[\left(\hat{\alpha}(\tau^2) - \alpha(\tau^2) \right)^4]$$

$$\leq E[\left(M_T \right)^4]$$

By a Poisson splitting argument, 

$$M_T {\buildrel d \over =} \frac{1}{n} \sum \limits_{i=1}^{N^1 + N^2} \gamma_i h_i$$

where $\gamma_i$ are i.i.d. Rademacher coin flips, and $h_i$ are i.i.d. draws from the distribution of $h$.

Hence,

$$E[\left(M_T \right)^4] = \frac{1}{n^4} E\left [ \sum \limits_{i=1}^{N^{tot}} \gamma_i h_i \right]$$

where $N^{tot} \sim Poisson(2n)$.

Let $\kappa := E[h_i^4]$, $\sigma^2 := E[h_i^2]$. Then, we can compute conditionally on $N^{tot}$ that

$$E\left[ \sum \limits_{i=1}^{N^{tot}} \gamma_i h_i | N^{tot}\right] = N^{tot} \kappa + 3 N^{tot} (N^{tot} - 1)\sigma^4$$

where other moments cancel out because $s_i$ is symmetrized. Since $E[N^{tot}] = 2n$ and $E[{N^{tot}}^2] = 4n^2 +2n$, we arrive at the result:

$$\frac{1}{n^4} E\left[ \sum \limits_{i=1}^{N^{tot}} \gamma_i h_i \right] = \frac{1}{n^4} \left[2 n \kappa + 3 \left(4n^2 + 2n - 2n \right) \sigma^4 \right]=\frac{2\kappa}{n^3} + \frac{12 \sigma^4}{n^2}$$

This completes the moment bound. We may now return to the tail bound lemma. 

\subsubsection{Tail bound}

The potential type I Error overshoot, which we needed to compute, was bounded by

$$ \int \limits_{x= 2.5\%}^{\infty} xP(\hat{\alpha}(\tau^2)-\alpha(\tau^2) > x) dx \leq \int \limits_{x = 2.5\%}^{\infty} x \frac{E[(\hat{\alpha}(\tau^2) - \alpha(\tau^2) )^4]}{x^4} = \int \limits_{x=2.5\%}^\infty \frac{ \frac{2\kappa}{n^3} + \frac{12\sigma^4}{n^2}}{x^3}$$

$$\frac{ \frac{2\kappa}{n^3} + \frac{12\sigma^4}{n^2}}{2*(2.5\%)^2} $$

\end{subsection}
\fi
%%% END REMOVE %%%

==> archive/scratch.tex <==
\begin{theorem}[T-net]\label{thm:main}
Let $\set{P_{\eta(\theta)} : \theta \in R^d}$ be 
an exponential family and
$\eta : R \mapsto \Xi$ is 
twice-continuously differentiable,
where $H \subseteq \R^d$ is a tile 
with a grid point $\theta_0 \in \R^d$ associated with it.
Further let $\set{p_m}_{m=1}^M \subseteq \R^d$ 
denote the points whose convex hull is $H$.
Let $(x,\theta) \mapsto F_{\theta}(x)$
be any function that is 
twice-continuously differentiable with respect to 
$\theta \in H$ and
define $f(\theta) := \EEE_{\theta}\br{F_{\theta}(X)}$
where $X \sim P_{\eta(\theta)}$.
Let $X_1,\ldots, X_n \sim P_{\eta(\theta_0)}$
be i.i.d. samples.
Fix any $\delta_1, \delta_2 \in [0,1]$.
Suppose the following assumptions hold:
\begin{enumerate}

% 0th order estimator
\item\label{ass:main-0th} 
There exists an estimator $\hat{U}_0$ 
depending on $\set{X_i}_{i=1}^n$ such that 
\begin{align}
    \prob_{\eta(\theta_0)}
    \br{\hat{U}_0 \geq f(\theta_0)} \geq 1-\delta_1
    \label{eq:0th-desire}
\end{align}

% 1st order estimator
\item\label{ass:main-1st} 
There exists estimators $\hat{\Delta}_m$
for $m=1,\ldots, M$ 
depending on $\set{X_i}_{i=1}^n$ such that 
\begin{align}
    \prob_{\eta(\theta_0)}
    \br{\nabla f(\theta_0)^\top v_m \leq \hat{\Delta}_m}
    \geq 
    1-\delta_2
    \label{eq:1st-desire}
\end{align}
where $v_m := p_m - \theta_0$.

% 2nd order estimator
\item\label{ass:main-2nd}
There exists a convex function $v \mapsto U_R(v)$,
which may depend on the tile $H$,
such that for any $v \in H-\theta_0$,
\begin{align}
    \int_0^1 (1-\alpha) 
    v^\top \nabla^2 f(\theta_0+\alpha v) v
    \, d\alpha
    &\leq
    U_R(v)
    \label{eq:2nd-desire}
\end{align}

\end{enumerate}
Then, 
\begin{align}
    \hat{U}
    :=
    \hat{U}_0
    +
    \max\limits_{m=1}^M
    \br{%
        \hat{\Delta}_m
        +
        U_R(v_m)
    }
    \label{eq:upper-bound}
\end{align}
satisfies
\begin{align}
    \prob_{\eta(\theta_0)}\br{\hat{U} \geq f(\theta)} \geq 1-\delta
    \quad , \quad \forall \theta \in H
    \label{eq:upper-bound-desire}
\end{align}
where $\delta := \delta_1 + \delta_2$.

\end{theorem}

% BEGIN: MOVE TO APPENDIX %
\begin{proof}
By the properties of exponential family
and that
$\eta(\theta)$ and $F_{\theta}(x)$
are twice-continuously differentiable
in $\theta$,
$f(\theta)$ is also twice-continuously differentiable.
Fix any $\theta$ and define $v := \theta-\theta_0$.
Then, a second-order Taylor expansion of $f(\theta)$ around $\theta_0$ gives
\begin{align*}
    f(\theta)
    &=
    f(\theta_0)
    +
    \nabla f(\theta_0)^\top v
    +
    \int_0^1 (1-\alpha) 
    v^\top 
    \nabla^2f(\theta_0+\alpha v)
    v
    d\alpha
\end{align*}

Let $\hat{U}_1 := \hat{U} - \hat{U}_0$.
By Assumption~\ref{ass:main-0th},
it suffices to show that
\begin{align}
    \prob_{\eta(\theta_0)}\br{
    \hat{U}_{1} \geq 
    \nabla f(\theta_0)^\top v +
    \int_0^1 (1-\alpha) 
    v^\top \nabla^2 f(\theta_0+\alpha v) v d\alpha } 
    \geq 
    1-\delta_2 
    \label{eq:1st-2nd-desire}
\end{align}
By Assumption~\ref{ass:main-2nd},
it suffices to show 
\begin{align*}
    \prob_{\eta(\theta_0)}\br{
    \hat{U}_1 \geq
    \sup\limits_{v\in H-\theta_0}
    \br{
        \nabla f(\theta_0)^\top v + U_R(v)
    }
    }
    \geq
    1-\delta_2
\end{align*}
Note that the sup is attained at some $v_m \equiv p_m-\theta_0$
by convexity.
Let $m^*$ be such that $v_{m^*}$ attains the sup.
Then,
\begin{align*}
    \prob_{\eta(\theta_0)}\br{
    \hat{U}_1 \geq 
    \nabla f(\theta_0)^\top v_{m^*} + U_R(v_{m^*})
    }
    &\geq
    \prob_{\eta(\theta_0)}\br{
    \hat{\Delta}_{m^*} \geq 
    \nabla f(\theta_0)^\top v_{m^*}
    }
    \\&\geq
    1-\delta_2
\end{align*}
where the last inequality follows by Assumption~\ref{ass:main-1st}.
\end{proof}
% END: MOVE TO APPENDIX %

\begin{remark}
The point $\theta_0$ associated with the tile $H$
in Theorem~\ref{thm:main}
need not be in 
$H$ or even $\Theta$, though it is wise
to choose $\theta_0 \in H$ whenever possible.
\end{remark}

Theorem~\ref{thm:main} gives a general way to construct
\emph{T-nets} for a large class of 
estimands.
The following corollaries extend this theorem
for studying a collection of estimands
and a collection of tiles.

\begin{corollary}\label{cor:main}
Let $\set{P_{\eta} : \eta \in \Xi}$ 
be a collection of distributions as in Theorem~\ref{thm:main}.
Let $\set{R_i}_{i=1}^I$, $\set{\theta_i}_{i=1}^I$ 
be a platten for 
a compact grid space $\Theta \subseteq \R^d$.
Let $\set{(x,\theta) \mapsto F_{\theta,i}(x)}_{i=1}^I$
be any collection of functions that are 
twice-continuously differentiable with respect to $\theta$
and define $f_i(\theta) := \EEE_{\theta}\br{F_{\theta,i}(X)}$
where $X \sim P_{\eta(\theta)}$.
Let $X_1^i,\ldots, X_{n_i}^i \sim P_{\eta(\theta_i)}$
be i.i.d. samples for every $i=1,\ldots, I$.
Fix any $\delta_1^i, \delta_2^i \in [0,1]$ 
for every $i=1,\ldots, I$.
Suppose that for every $i=1,\ldots, I$,
the inputs
$\set{X_j^i}_{j=1}^{n_i}, f_i(\theta),R_i,\theta_i,\delta_1^i, \delta_2^i$ 
satisfy the conditions in Theorem~\ref{thm:main}.
Then, 
there exists a collection of estimators $\set{\hat{U}_i}_{i=1}^I$,
where each $\hat{U}_i$ depends on 
$\set{X_j^i}_{j=1}^{n_i}$,
such that for all $i=1,\ldots, I$,
\begin{align}
    \prob_{\eta(\theta_i)}\br{\hat{U}_{i} \geq f_{i}(\theta)} \geq 1-\delta_i
    \quad \forall \theta \in H_i
    \label{eq:upper-bound-desire-tiles}
\end{align}
where $\delta_i := \delta_1^i + \delta_2^i$.
\end{corollary}

% BEGIN: MOVE TO APPENDIX %
\begin{proof}
The proof follows immediately from 
repeated applications of Theorem~\ref{thm:main}.
\end{proof}
% END: MOVE TO APPENDIX %

\begin{corollary}\label{cor:combined}
Under the setting of Corollary~\ref{cor:main},
define 
\begin{align*}
    f(\theta) 
    &:= 
    \max\limits_{i : \theta \in H_i} f_i(\theta) \\
    \hat{U}(\theta) 
    &:= 
    \max\limits_{i : \theta \in H_i} \hat{U}_i \\
    \delta 
    &:= 
    \max\limits_i \delta_i
\end{align*}
Then,
\begin{align*}
    \prob\br{\hat{U}(\theta) \geq f(\theta)} \geq 1-\delta
    \quad \forall \theta \in \Theta
\end{align*}
\end{corollary}

% BEGIN: MOVE TO APPENDIX %
\begin{proof}
For any fixed $\theta \in \Theta$,
let $i^*$ be the index which maximizes $f_i$, so that $f(\theta) = f_{i^*}(\theta)$.
Then,
\begin{align*}
    \prob\br{\hat{U}(\theta) \geq f(\theta)}
    &=
    \prob\br{\hat{U}(\theta) \geq f_{i^*}(\theta)}
    \geq
    \prob\br{\hat{U}_{i^*} \geq f_{i^*}(\theta)}
    \geq
    1-\delta_{i^*}
    \geq
    1-\delta
\end{align*}
\end{proof}
% END: MOVE TO APPENDIX %

\begin{remark}\label{rem:piecewise}
Corollary~\ref{cor:combined}
is especially useful when one is interested
in a function $(x,\theta) \mapsto F_\theta(x)$
that is piece-wise twice-continuously differentiable,
i.e. $\theta \mapsto F_{\theta}(x)$ is 
twice-continuously differentiable in the interior 
of each tile $R_i$ (without loss of generality).
Since the interior of tiles are disjoint, the only possible
overlap of tiles are at the boundaries,
which is exactly where $\theta\mapsto F_{\theta}(x)$ 
may not be twice-continuously differentiable.
Along the boundaries then, $f(\theta)$ 
is the ``worst'' possible value
and $\hat{U}(\theta)$ chooses the correspondingly
most conservative upper bound estimator.
\end{remark}

Before closing this section,
we present a few lemmas that will be useful
for the later sections.

\begin{lemma}\label{lem:0th-hoeffding}
    Let $X_i \sim P$ 
    for $i=1,\ldots, n$
    be i.i.d. random variables
    bounded in [a,b] and $\mu := \EEE_P\br{X}$.
    Then, 
    \begin{align*}
        \prob\br{
        \hat{U}_0 \geq \mu
        }
        &\geq 1-\delta
    \end{align*}
    where 
    \begin{align*}
        \hat{U}_0
        &:=
        \frac{1}{n}
        \sum\limits_{i=1}^n X_i
        +
        \sqrt{\frac{(b-a) \log\pr{\frac{1}{\delta}}}{2n}}
    \end{align*}
\end{lemma}

% BEGIN: MOVE TO APPENDIX %
\begin{proof}
    The proof follows immediately by Hoeffding's inequality.
\end{proof}
% END: MOVE TO APPENDIX %

\begin{lemma}\label{lem:unbiased}
Let $X_1,\ldots, X_n \sim P$ be i.i.d.\ samples
and $G(P) \in \R^d$ be any estimand.
Suppose the following assumptions hold:
\begin{enumerate}
\item\label{ass:lem-1st-unbiased}
There exists a function 
$U(x)$ such that $U(X)$ is unbiased for $G(P)$
where $X \sim P$.
\item There exists $v \mapsto V(v)$ 
such that $\var\br{v^\top U(X)} \preceq V(v)$.
\end{enumerate}
Then, for any $\delta \in [0,1]$ and $v \in \R^d$,
\begin{align*}
    \hat{\Delta}
    &:=
    \frac{1}{n} \sum\limits_{i=1}^n
    U(X_i)^\top v
    +
    \sqrt{\frac{V(v)}{n}\pr{\frac{1}{\delta}-1}}
\end{align*}
satisfies
\begin{align*}
    \prob\br{
    \hat{\Delta} \geq G(P)^\top v
    }
    &\geq
    1-\delta
\end{align*}

\end{lemma}

\begin{proof}
By Cantelli's inequality and 
Assumption~\ref{ass:lem-1st-unbiased},
the result holds for $V(v) = \var\br{v^\top U(X)}$,
so it must hold for any $V(v) \geq \var\br{v^\top U(X)}$.
\end{proof}

\begin{lemma}\label{lem:1st}
Under the setup of Theorem~\ref{thm:main},
assume that there exists an unbiased 
random variable
for $\nabla f(\theta_0)$ of the form
\begin{align*}
U_{\nabla f}(X)
&:=
B(\theta_0) + 
(F_{\theta_0}(X)-\varphi(\theta_0)) s_{\theta_0}(X)
\end{align*}
for some $B$ and $\varphi$,
where 
$s_{\theta_0}(x) = \nabla_\theta \log p_{\eta(\theta_0)}(x)$.
Suppose that 
\[
C := \sup\limits_{x}\abs{F_{\theta_0}(x)-\varphi(\theta_0)}
< \infty
\]
Then, for any $\delta \in [0,1]$ and $v \in \R^d$,
\begin{align*}
\hat{\Delta}
&:=
\frac{1}{n}
\sum\limits_{i=1}^n U_{\nabla f}(X_i)^\top v
+
C
\sqrt{\frac{v^\top \var_{\eta_0}\br{{s_{\theta_0}(X)}} v}{n} \pr{\frac{1}{\delta}-1}}
\end{align*}
satisfies
\begin{align*}
    \prob\br{\hat{\Delta} \geq \nabla f(\theta_0)^\top v}
    &\geq
    1-\delta
\end{align*}
\end{lemma}

\begin{proof}
We first compute a bound on the variance of $U_{\nabla f}(X)$ when $X \sim P_{\eta(\theta_0)}$.
For any $v \in \R^d$
{\small
\begin{align*}
    \var_{\eta(\theta_0)}\br{v^\top U_{\nabla f}(X)}
    &\leq
    \EEE_{\eta(\theta_0)}
    \br{(F_{\theta_0}(X)-\varphi(\theta_0))^2 
    \pr{v^\top s_{\theta_0}(X)}^2}
    \\&\leq
    \sup\limits_{x}(F_{\theta_0}(x)-\varphi(\theta_0))^2
    \cdot 
    v^\top \var_{\eta(\theta_0)}\br{s_{\theta_0}(X)} v
    \\&=
    C^2 
    v^\top \var_{\eta(\theta_0)}\br{s_{\theta_0}(X)} v
\end{align*}
}

The desired claim holds by Lemma~\ref{lem:unbiased},
with $P \equiv P_{\eta(\theta_0)}$,
$G(P) \equiv \nabla f(\theta_0)$,
$U \equiv U_{\nabla f}$,
and 
$V(v) \equiv C^2 
v^\top \var_{\eta(\theta_0)}\br{s_{\theta_0}(X)} v$.
\end{proof}

\begin{lemma}\label{lem:2nd}
Under the setting of Theorem~\ref{thm:main},
consider
\begin{align}
    G(\theta)
    &=
    \int F_\theta(x)
    \nabla^2 p_{\eta(\theta)}(x) 
    \,
    d\mu(x)
    \label{eq:2nd-upper}
\end{align}
Let $s_{\theta}(x) := \nabla_\theta \log p_{\eta(\theta)}(x)$
and $s_{\theta, k}(x)$ be the kth component of $s_{\theta}(x)$.
Let $T$ be the sufficient statistic.
Suppose that
\begin{align*}
    C_1 &:= 
    \sup\limits_{\theta \in H} 
    \sup\limits_{x}
    \abs{F_\theta(x)-\EEE_{\eta(\theta)}\br{F_\theta(X)}}
    < \infty
    \\
    C_2 &:=
    \sup\limits_{\theta \in H} 
    \sup\limits_{x}
    \abs{F_\theta(x)-\varphi(\theta)}
    < \infty
\end{align*}
for any given $\varphi$.
Define
\begin{align}
    \tilde{U}_R(v)    
    \label{eq:UR-wiggle}
    &:=
    \tilde{U}_{R,1}(v) + \tilde{U}_{R,2}(v) 
    \\
    \tilde{U}_{R,1}(v)
    &:=
    C_1 \sup\limits_{\theta \in H} 
    \br{
        v^\top \var_{\eta(\theta)}\br{s_{\theta}(X)} v
    }
    \\
    \tilde{U}_{R,2}(v)
    &:=
    C_2
    \norm{v}^2
    \sum\limits_{k} 
    \sup\limits_{\theta \in H}
    \br{%
        \opnorm{\nabla^2 \eta_k(\theta)}
        \sqrt{\var_{\eta(\theta)}\br{T(X)}}
    }
\end{align}
Define
\begin{align*}
    U_R(v)
    :=
    \frac{1}{2} \tilde{U}_R(v)
\end{align*}
Then, $U_R$ is convex and for any $v \in H-\theta_0$
and $\theta \in H$,
\begin{align*}
    v^\top G(\theta) v
    &\leq
    \tilde{U}_R(v)
\end{align*}
In particular,
\begin{align*}
    \int_0^1
    (1-\alpha) v^\top G(\theta_0+\alpha v) v 
    \,d\alpha
    \leq
    U_R(v)
\end{align*}
\end{lemma}

\begin{proof}

It is easy to see that $U_R$ is convex.
We prove the rest of the claim.

We first simplify $\nabla^2 p_{\eta(\theta)}(x)$.
\begin{align*}
    \nabla^2 p_{\eta(\theta)}(x)
    &=
    (\eta'(\theta))^\top 
    \nabla^2_{\eta} p_{\eta(\theta)}(x) 
    \eta'(\theta)
    +
    \sum\limits_{k} 
    \frac{\partial p_{\eta(\theta)}(x)}{\partial \eta_k} 
    \nabla^2 \eta_k(\theta)
    \\
    \nabla^2_\eta p_{\eta}(x)
    &:=
    (T(x)-\nabla_\eta A(\eta))
    (T(x)-\nabla_\eta A(\eta))^\top p_\eta(x)
    -
    \nabla_\eta^2 A(\eta) p_\eta(x)
\end{align*}
Let $\nu(\theta) := \EEE_{\eta(\theta)}\br{F_\theta(X)}$.
Note that we may subtract $F_\theta(x)$ 
by $\nu(\theta)$
in the integral on the right side of (\ref{eq:2nd-upper}).
It is easy to see that for any $\eta$,
\begin{align*}
    -C_1 \var_\eta\br{T(X)}
    \preceq
    \int (F_{\theta}(x)-\nu(\theta)) 
    \nabla^2_\eta p_{\eta}(x) 
    \, d\mu(x)
    \preceq
    C_1 \var_\eta\br{T(X)}
\end{align*}

Note that if $A \preceq B$
for any square matrices $A, B$,
then we must have that for any matrix $S$,
$S^\top A S \preceq S^\top B S$.
This is because $A \preceq B$
if and only if $B-A$ is positive semi-definite,
and $S^\top (B-A) S$ is clearly positive semi-definite as well.
Rearranging, we have our claim.
Hence, 
\begin{align*}
    -C_1 \var_\eta\br{s_{\theta}(X)}
    &\preceq
    (\eta'(\theta))^\top
    \int (F_\theta(x)-\nu(\theta)) 
    \nabla_\eta^2 p_{\eta}(x) d\mu(x)
    \,
    \eta'(\theta)
    \\&\preceq
    C_1 \var_\eta\br{s_{\theta}(X)}
\end{align*}
This shows that
\begin{align}
    v^\top 
    G(\theta)
    v
    &\leq
    C_1 \,
    v^\top \var_{\eta(\theta)}\br{s_\theta(X)} v 
    \nonumber
    \\&\quad +
    \sum\limits_{k} 
    v^\top \nabla^2 \eta_k(\theta) v
    \int
    F_\theta(x)
    \frac{\partial p_{\eta(\theta)}(x)}{\partial \eta_k}
    \, d\mu(x)
    \label{eq:2nd-hessian}
\end{align}

Next, we bound the second term on the right side 
of (\ref{eq:2nd-hessian}).
Similarly as before, we may subtract
$F_\theta(x)$ by $\varphi(\theta)$
in (\ref{eq:2nd-hessian}).
Then, letting $t_{\theta,k}(x) := T_k(x) - \frac{\partial A(\eta(\theta))}{\partial \eta_k}$,
\begin{align*}
    \int \abs{F_\theta(x)-\varphi(\theta)} 
    \abs{t_{\theta,k}(x)} p_{\eta(\theta)}(x) 
    \, d\mu(x)
    &\leq
    C_2 \int \abs{t_{\theta,k}(x)} p_{\eta(\theta)}(x) 
    \, dx
    \\&\leq
    C_2
    \pr{\int t_{\theta,k}(x)^2 p_{\eta(\theta)}(x)
    \, dx}^{1/2}
    \\&=
    C_2
    \sqrt{\var_{\eta(\theta)}\br{T_k(X)}}
\end{align*}

Hence, we have that the left side of (\ref{eq:2nd-hessian})
is further uniformly (over $\theta \in H$) bounded above by
\begin{align*}
    \tilde{U}_{R,1}(v)
    +
    C_2
    \sum\limits_{k}
    \sup\limits_{\theta \in H}
    \br{%
        \abs{v^\top \nabla^2 \eta_k(\theta) v}
        \sqrt{\var_{\eta(\theta)}\br{T_k(X)}}
    }
    \leq
    \tilde{U}_R(v)
\end{align*}
This immediately shows the desired claim.

\end{proof}

\begin{corollary}\label{cor:lem:2nd}
Under the setting of Lemma~\ref{lem:2nd},
assume that
\begin{align*}
    \nabla^2 f(\theta)
    &:=
    H(\theta)
    +
    G(\theta)
\end{align*}
for some $H$.
Let 
\begin{align*}
    \tilde{H}(v)
    &:=
    \int_0^1 (1-\alpha) v^\top H(\theta_0+\alpha v) v
    \, d\alpha
\end{align*}
Assume further that there exists a convex function $K$
such that $\tilde{H}(v) \leq K(v)$.
Let
\begin{align*}
    U_R(v)
    &:=
    K(v) + \frac{1}{2} \tilde{U}_R(v)
\end{align*}
Then, $U_R$ is convex and for any $v \in H-\theta_0$,
\begin{align*}
    \int_0^1
    (1-\alpha) v^\top \nabla^2 f(\theta_0+\alpha v) v
    \, d\alpha
    \leq
    U_R(v)
\end{align*}
\end{corollary}

\begin{proof}
It is immediate that $U_R$ is convex.
Lemma~\ref{lem:2nd} shows that
\begin{align*}
    \int_0^1 (1-\alpha)
    v^\top G(\theta_0+\alpha v) v
    \, d\alpha
    \leq 
    \frac{1}{2} \tilde{U}_R(v)
\end{align*}

where $\tilde{U}_R(v)$ is defined as in \ref{eq:UR-wiggle} in Lemma ~\ref{lem:2nd}). 
This concludes the proof.
\end{proof}

\begin{remark}\label{rem:more-conservative}
In general, we can make $U_R(v)$ 
in Lemma~\ref{lem:2nd} even more conservative
by taking further upper bounds to make the computations more tractable.
\end{remark}

\begin{remark}
In Lemma~\ref{lem:2nd},
note that $\tilde{U}_{R,2}(v) = 0$ for any linear transformation $\eta$.
In particular, for the identity transformation, it simplifies to 
\begin{align*}
    U_R(v) = 
    \tilde{H}(v) + \frac{1}{2}\tilde{U}_{R,1}(v) = 
    \tilde{H}(v) +
    \frac{1}{2}
    \sup\limits_{\theta \in H} v^\top \var_{\eta(\theta)}\br{T(X)} v
\end{align*}
which can be further bounded above 
(see Remark~\ref{rem:more-conservative})
by the formula
\begin{align*}
    \tilde{H}(v) +
    \frac{1}{2}
    v^\top \sup\limits_{\theta \in H} \var_{\eta(\theta)}\br{T(X)} v
\end{align*}
where the sup is element-wise (along the diagonal).
\end{remark}

\section{Beyond Exponential Families, to Log-Concave Distributions}

The theory that we derive in Appendix A and  \cite{sklar:2022} assumed that our distributional family was an exponential family. This assumption led to simplicity and convenience, thanks to exponential family moment identities. In the general case, control over the derivatives of the target function may be more complicated to establish or altogether unclear. This section considers log-concave families, a large class which contains the exponential families. A family of densities indexed by $\theta$ is said to be log-concave if and only if the log-likelihood of the density $\log p(X,\theta)$, is concave in $\theta$. In the following subsections X, we derive a general approach to the log-concave case, and calculate relevant expressions for the logistic model as an example.

\subsection{CSE for general log-concave models}

There are 3 places in Section X where exponential family models were used. We shall substitute results for log-concave models in their place.

\begin{enumerate}
    \item Constructing an unbiased estimate of $\nabla f(\theta_i)$ in Line X
    \item Bounding the (co)variance (matrix) of this unbiased estimate in Line X
    \item Bounding $\nabla^2 f(\theta)$ uniformly over $R_i$, in Line X
\end{enumerate}

We address these respectively in the following 3 subsections X, Y, and Z.

\subsubsection{Unbiased Gradient Estimation with the Score Estimator}

To get an unbiased estimate of $\nabla f$, we may similarly apply the approach in Line X, but now using the log-concave density representation $dP(x) = e^{-g(x,\theta)}dx$ for some $g$ which is convex in $\theta$. Then, if $F_{\theta}(X)$ is an indicator variable that with parameter $\theta$ a false rejection has occurred,

$$f(\theta) = \int F_{\theta}(X) dP_{\theta}(X) = \int F_{\theta}(X)  e^{-g(x,\theta)}dx$$

$$\nabla f(\theta) = 
\int F_{\theta}(X) \left[ - \nabla g(x,\theta) e^{-g(x,\theta)} \right] dx 
= \int \left[ - F_{\theta}(X)\nabla g(x,\theta) \right] dP_{\theta}(x)$$

Hence, $$\widehat{\nabla f}_j = -\frac{1}{N_{sim}} \sum \limits_j F_{\theta}(X_j) \nabla g(X_j,\theta)$$

is an unbiased estimator of the gradient.

\subsubsection{Controlling the Variance of the Gradient Estimate}

Similarly, we may apply the arguments of Line X to bound 

$$Cov(\widehat{\nabla f}_j) 
\leq Cov(\nabla g(X_j,\theta))$$

Furthermore it turns that by a well-known identity for Fisher information, which holds under sufficient regularity, that we have

$$Cov(\nabla g(X_j,\theta)) = E[\nabla^2 g(X_j,\theta]$$

Thus, our problem is reduced to bounding the latter term. This term will also show up in the next subsection; we must assume knowledge of a bound. Ahead in Line X we will see that in the logistic regression case this becomes a straightforward expression.

\subsubsection{Bounding the Hessian}

Following line X, we will write

$$\nabla^2 f(\theta) = \nabla^2 \int F_{\theta}(X) dP(X)
=\int F_{\theta}(X) \nabla^2 dP(X)$$

Where we have assumed $F_{\theta}(X)$ is locally constant in $\theta$, which is true in the case of Type I Error and FDR.
The second derivative of the log-concave likelihood is 
$$\left(\nabla g \nabla g^T \right)e^{-g(\theta)} - 
\nabla^2 g(\theta) e^{-g(\theta)} \preccurlyeq \nabla g(\theta) \nabla g(\theta)^T e^{-g(\theta)} $$.

Where the inequality holds by convexity of $g$ and since $exp(\cdot)$ is strictly positive. Since this bound is always PSD, we have

$$\nabla^2 f(\theta) \preccurlyeq \int F_{\theta}(X) \nabla g(\theta) \nabla g(\theta)^T e^{-g(\theta)} dX \preccurlyeq \int  \nabla g(\theta) \nabla g(\theta)^T e^{-g(\theta)} dX$$

Which, similar to the previous subsection is equal to 

$$Cov(\nabla g(X,\theta)) = E[\nabla^2 g(X,\theta].$$

Thus, we again find ourselves needing to bound this quantity. Furthermore, unlike the previous occurrence, we will need to take a worst-case over the rectangle $H_j$. Fortunately, mathematical analysis is usually able to provide the necessary control. We give a concrete example in the next subsection, showing the relevant bounds for logistic regression

\subsection{Example: Logistic model}

The logistic model is commonly used for binary response data, with continuous covariates. For each response $i$, the success probability $p_i$ is modeled as

$$p_i = Pr(y_i = 1) = \frac{1}{1 + exp(- (x_i^T \beta))}$$ 

where $x_i$ is a vector of covariates and $\beta$ is the unknown parameter vector of the model. (Typically $x_{i,1}$ is identically set to 1, to allow for intercept estimation). 
Thus, given an observation vector $y$, the likelihood of the logistic model is

$$ 
\prod \limits_{i=1}^n 
\left( \frac{1}{1 + exp(-x_i^T\beta)} \right)^{y_i}
\left( \frac{exp(-x_i^T\beta)}{1 + exp(-x_i^T\beta)} \right)^{1-y_i}
$$

Taking a derivatives of the log-likelihood with respect to the unknown parameter vector $\beta$, we arrive the expression

$$\nabla_{\beta} LL = \sum \limits_{i=1}^n \left(y_i - p_i \right) x_i $$

Thus, our score-based gradient estimator for logistic regression is 

$$\widehat{\nabla f} = \frac{1}{N_{sim}} \sum \limits_{j = 1}^{N_{sim}} \sum \limits_{i=1}^n F_{j} \left(y_{ij} - p_{i} \right) x_{i}$$

Where, for Type I Error, $F_j$ is the indicator of a false rejection. Furthermore, to bound the expressions in Line X (above where we compute the inequality for $\nabla^2 f(\theta)$), we can arrive at the formula

$$\nabla^2 f \preccurlyeq E[\nabla^2 g] = E[-\nabla^2_{\beta} LL] = \sum \limits_{i=1}^n p_i \left(1 - p_i \right) x_i x_i^T$$

Finally, for expression Y, we maximize over $p_i \in H$. For a simple and conservative bound, we could use the fact that $p_i(1-p_i) \leq .25$, arriving at the bound for line X:

$$\sup \limits_{\theta \in H} \nabla^2 f(\theta) \preccurlyeq \frac{1}{4} \sum \limits_{i=1}^n x_i x_i^T$$

In the setting where the covariates $x_i$ are known or set a priori, we can directly apply this formula to Line X. We caution that if sampling were adaptive in a fashion that is responsive to outcomes, one may not be able to condition on the sequence of $x_i$ as we have done.

\subsection{(Mike's note: the following is TOO COMPLICATED. KEEP OUT OF PAPER and SOFTWARE.) Extending arguments to give a Hessian bound}

The Hessian term in a Taylor expansion along a line from the center-point $\theta_0$ to $\theta + v$ is:

$$ \int \limits_{0}^{1} (1-\alpha) v^T \nabla^2 f v d\alpa $$

We may now write

$$\nabla^2 f = \int F(X) [(T(X) - \nabla A(\theta))(T(X) - \nabla A(\theta))^T - \nabla^2 A(\theta)] dP(X)$$

where $F$ would be a binary indicator of false rejection, for type I Error validation. As in the original thesis, we will split this into 

$$ \int - F(X) \nabla^2 A(\theta) dP(X) \preccurlyeq  \nabla^2 f \preccurlyeq \int F(X) [(T(X) - \nabla A(\theta))(T(X) - \nabla A(\theta))^T] dP(X)$$


[insert arguments]

we conclude that it suffices to control quantities such as:

$$\sup \limits_{\theta \in H, v \in H - \theta_0} \int F(X) v^T \nabla^2 A_{\tau}(\theta) v  dP(X)$$ 

and

$$\sup \limits_{\theta \in H, v \in H - \theta_0} \int F(X) v^T [(T(X) - \nabla A(\theta))(T(X) - \nabla A(\theta))] v  dP(X)$$ $$

we can upper bound these respectively by the more extreme quantities:

$$\sup \limits_{\theta \in H, v \in H - \theta_0} \int v^T \nabla^2 A_{\tau}(\theta) v  dP(X)$$

$$ = $$

$$\sup \limits_{\theta \in H, v \in H - \theta_0} \int v^T [(T(X) - \nabla A(\theta))(T(X) - \nabla A(\theta))] v  dP(X)$$

Note that these two expressions are now actually equal.

How to handle this sup?

There is good news: as shown in the previous section, our quantities of interest take the form 

$$\sup \limits_{\theta \in H} E_{\theta}[\tau ^T c]$$

(where the c term involves $v_i$ and $A(\theta)$).

The key insight is that \textit{this is a smooth function of $\theta$, with a bounded estimator}. The bounded estimator is $F(X) = \frac{1}{K} \sum \tau_k^T c$, and we may take $G = 0$. Hence, techniques from the following section can be applied to derive a Taylor expansion for uniform control over the rectangle.

The result is that for each corner $v$, we may apply the methods of the next section to gain uniform control over 

$$\sup \limits_{\theta \in H} v^T \int \nabla^2 A_{\tau}(\theta) v (X)$$.





%%% BEGIN: LEGACY %%%
% Everything has been ported over to the main results
% with a more consistent notation and 
% fully generalized.
% There's really no need for this anymore.
\section{Estimation of general quantities and FDR control}

We now further extend our methods to apply to general estimators. We will show that, given a locally smooth target function $G(\theta)$ - which could be the mean of our exponential family distribution, or an expected improvement in a metric comparing treatments, or some other functional of our exponential family - that if our estimator $\hat{G} = F(X)$\todojames{kinda feel weird saying $F_\theta(X)$ is an estimator cuz it depends on the parameter} is bounded, we can give computational bounds on $F$'s accuracy - such as its bias and mean squared error functions, $B(\theta)$ and $MSE(\theta)$.

Similar to our previous treatment of intersection null hypotheses in Section X, we may further write $F$ and $G$ as $F_{H(\theta)}(X)$ and $G_{H(\theta)}(\theta)$, respectively, which may take a different character on different pre-identified intersection null hypotheses; this generalization poses no issue, as we will be splitting the space using tiles along null hypothesis boundaries, and handling them separately. So, in the following sections, we suppress the notation of this dependence of $F$ on $\theta$, as we can safely localize our attention to each intersection hypothesis on its own. The advantage of this generalization, is that our results will immediately also apply to bounding quantities such as the FDR: to achieve that, we would $G$ constant and take $F = \frac{\sum \limits_i \mathbbm{1}_{\theta_i \in H_0} \mathbbm{1}_{rej_i}}{1 \vee \sum \limits_i \mathbbm{1}_{rej_i}}.$

Our analysis will track the previous sections, with minor modifications. Here is a list of these modifications (just for now, while the base section remains unwritten; we can expand this out in a full copy later once the base section is complete).

\begin{enumerate}
    \item Whereas before we performed a Taylor Expansion on the smooth Type I Error function, now we perform a Taylor Expansion on
    $$f( \theta) = E\left[F(X) - G(\theta)\right].$$ So, for an estimator $F(X)$ of $G(\theta)$, $f$ is the bias as a function of $\theta$. (Copying the previous treatment, we may simply write out the same exact Taylor Expansion, or refer to the formula, with zero changes except for the definition of f.)
    \item 0'th order Monte Carlo term: for each $\theta_i$ we still have the unbiased estimator,
    
    $$\widehat{f(\theta_i)}_k := F(X_k) - G(\theta_i)).$$
    
    Notice however that the confidence intervals approach in Section X, using Clopper-Pearson, no longer works as the distribution of $\sum F_i$ is not necessarily binomial. Instead, we shall construct a confidence interval, leveraging only the boundedness of our estimator. For this, we may use Hoeffding's inequality (see page 6 of http://cs229.stanford.edu/extra-notes/hoeffding.pdf). (Note: if it turns out that this is too shitty, we could look into other things, but it's probably going to be good enough and also pretty hard to beat this).
    \item Our equation for the gradient $\nabla f$ is slightly altered: we now have
    \begin{align*}
        \nabla f(\cdot) 
        &= 
        -\nabla G(\cdot) + \nabla P_{(\cdot)} F(X) 
        =
        -\nabla G(\cdot) + \nabla \int F(X) dP_{(\cdot)} dX
        \\&= 
        -\nabla G(\cdot) + \int F(X) (T(X) - \nabla A(\cdot)) dP_{(\cdot)}
    \end{align*}
    The result is that
    $$\widehat{\nabla f_{\theta_j}} := -\nabla G(\theta_j) + \frac{1}{K}\sum \limits_{k=1}^K F(X_k)(T(X_k) - \nabla A(\theta_j))$$
    is an unbiased estimator of the gradient.
    \item But wait! Before continuing further to the gradient confidence interval, we can actually back up make a general improvement to the techniques of the original thesis, by first centering $F$ with respect to our bound. If we know $F \in [a,b]$, then we may instead center it in its interval by taking $F^*(X) := F(X) - (b - a)/2$ so that $F^*(X) \in [-C, C]$ where $C = (b-a)/2$. Going back to the integral, where we had
    
     $$\nabla f(\cdot) = -\nabla G(\cdot) + \int F(X) (T(X) - \nabla A(\cdot)) dP_{(\cdot)}$$ 
     
     $$ = -\nabla G(\cdot) + \int F^*(X) (T(X) - \nabla A(\cdot)) dP_{(\cdot)} + \int [(b-a)/2] (T(X) - \nabla A(\cdot)) dP_{(\cdot)}$$
     
      $$ = -\nabla G(\cdot) + \int F^*(X) (T(X) - \nabla A(\cdot)) dP_{(\cdot)} + 0$$
    
     this in fact will offer us a different unbiased estimator, and we will consequently find a smaller bound on its variance
     
     $$\widehat{\nabla f_{\theta_j}} := -\nabla G(\theta_j) + \frac{1}{K}\sum \limits_{k=1}^K F^*(X)(T(X) - \nabla A(\cdot))$$
 
    Compared to the original thesis document, I believe this reduces our cantelli bound width by a whole entire factor of 2! (James, please read the below and tell me if I've just been up too late?)
    
    \item Now, the confidence interval for the new gradient estimate: note that comparing this unbiased gradient estimate to the simpler estimator of Section X, this generalized form has essentially been multiplied by $F(X)$ (and without a restriction on the set of integration). As before, we shall seek to bound the variance of this expression, so that we may use a Cantelli bound.
   
    $$= Var_{\theta_j}\left[(F^*(X) v^T(T(X) - \nabla A(\theta_j))\right]$$
    
    $$= E_{\theta_j}\left[(F^*)^2 (v^T(T(X) - \nabla A(\theta_j))^2\right] - E_{\theta_j}\left[F^* v^T(T(X) - \nabla A(\theta_j\right]^2$$
    
    $$\leq E_{\theta_j}\left[(F^*(X))^2 (v^T(T(X) - \nabla A(\theta_j)))^2 \right] $$
    
    $$\leq C^2 E_{\theta_j} \left[(v^T(T(X) - \nabla A(\theta_j)))^2\right ] \leq C^2 v^T I_{\tau_{max}}v$$
    
    Hence, it is sufficient to simply simply inflate $I_{\tau_{max}}$ in equation X by a factor of $C^2$. (Note that this translation argument already improves the original thesis bound! Since we can take C = 1/2 after centering)
    
    \item The Hessian as a function of $\theta_j$: %We may attempt to generalize this as well, continuing with the centering technique from above, although we do not this time get a clean improvement. Let $F^{**} := F(X) - E_{\cdot}[F(X)]$. Then by an identical argument to the above that we had for $F^*$, we will have
    We have FIXX THISSSS!!!! THERE WAS AN ERROR BEFORE, and the below is not longer a correct argument when we "choose f to set an integral to zero"!
    
    $$\nabla f = -\nabla G(\cdot) + \int F(X) (T(X) - \nabla A(\cdot)) dP_{(\cdot)}(X)$$
    
    we now take
    
    $$\nabla^2 f (\cdot) = -\nabla^2 G(\cdot) + \int F(X) (T(X) - \nabla A(\cdot)((T(X) - \nabla A(\cdot))^T dP_{(\cdot)}(X) + \int F(X) (- \nabla^2 A(\cdot))^2 dP_{(\cdot)}(X)$$
    
    $$= -\nabla^2 G(\cdot) + \int F(X) (T(X) - \nabla A(\cdot)((T(X) - \nabla A(\cdot))^T dP_{(\cdot)}(X) + 0$$
    
    by our choice of $F$. Then, 
    
    $$v^T \nabla^2 f (\cdot)v \leq -v^T \nabla^2 G(\cdot) v + \|F\|_{\infty} v^T I(\cdot) v $$
    
    $$v^T \nabla^2 f (\cdot)v \geq -v^T \nabla^2 G(\cdot) v - \|F\|_{\infty} v^T I(\cdot) v$$
    
    The result is that
    
    $$ - \|F\|_{\infty} I(\cdot) - \nabla^2 G \preccurlyeq \nabla^2 f(\cdot) \preccurlyeq \|F\|_{\infty} I(\cdot) - \nabla^2 G $$
    
    Note that if $F$ lies in $[0,C]$, then $\|F\|_{\infty} \leq C$; so in the worst case, in the original Type I Error application where G = 0 and C = 1, we recover our original bound from the original thesis \cite{sklar:2022}.
    
    %and if we have additional information which can restrict $F^{**}$, then a slightly smaller Hessian bound is permitted. [Note: perhaps we might be able to leverage some knowledge about F** to do this, since we can WLOG assume that $E_{\theta_j}F(X)$ lies in the confidence set from the basic Monte Carlo. However, we'll still have to control the worst case over $H_j$ somehow.]
    
    
    
\end{enumerate}

\begin{subsection}{Mean-Squared-Error}

In the previous section, we showed how to bound $$E_{(\cdot)}\left[F(X) - G(\cdot)\right]$$ where $F(X)$ is a known estimator and $G(\cdot)$ is a known function. Unfortunately we cannot apply these results directly if our goal is to understand the MSE of the estimator, since MSE takes the form

$$f^{MSE}(\cdot) := E_{(\cdot)}\left[(F(X) - G(\cdot))^2\right] =  E_{(\cdot)}\left[F(X)^2 + G(\cdot)^2 - 2 F(X)G(\cdot) \right]$$

because the expectation of the cross-term $F(X)G(\cdot)$ is only known if the bias function is known.

Here we list modifications to the previous steps, which will allow us to extend control to this case:

\begin{enumerate}
    \item $$f^{MSE}(\theta) = E\left[F(X) - G(\theta)\right].$$ So, (copying the previous treatment, we may simply write out the same exact Taylor Expansion, or refer to the formula, with zero changes except for the definition of f.)
    \item 0'th order Monte Carlo term: for each $\theta_j$ we have the unbiased estimator,
    $$\widehat{f(\theta_j)}_k := (F(X_k) - G(\theta_j))^2.$$ Using boundedness of $F$, we may apply Hoeffding \ldots (write this out)
    \item 1st order Monte Carlo estimate for the gradient of MSE at $\theta_j$: since
    $$\nabla f^MSE (\cdot) = \int (F(X) - G(\cdot))^2 (T(X) - \nabla A(\cdot))dP_{(\cdot)}(X) + \int 2 \nabla G(\cdot))(G(\cdot) - F(X)) dP_{(\cdot)}(X)$$
    
     $$\nabla f^MSE (\cdot) = \int (F(X) - G(\cdot))^2 (T(X) - \nabla A(\cdot))dP_{(\cdot)}(X) +  2 \nabla G(\cdot))(G(\cdot) - F(X)) $$
     
     Which permits the unbiased estimator,
     
     $$ \widehat{\nabla f^{MSE} (\theta_j)} =  \frac{1}{K}\sum \limits_{k=1}^K 2 \nabla G(\theta_j )(G(\theta_k)- F(X_k)) + (T(X_k) - \nabla A(\theta_j))(G(\theta_j)- F(X_k))^2$$
     \item In light of the previous centering arguments, the following may be improvable, but let's just put it down regardless:
     
     We shall again argue by Cantelli; for this we need variance estimate for linear evaluations of our estimate of the true gradient, 
     $$Var(v^T \widehat{\nabla f^{MSE}(\theta_k)}).$$
     
     If on rectangle $j$ our estimator $F$ is bounded in $[a,b]$, then this implies $(G(\theta_j)- F(X_k))$ is bounded in $[c,d].$ Let $C := max(|c|, |d|).$ Then, we estimate the variance of a single first-order summand, as
     
     $$Var_{\theta_j}\left[v^T (G(\theta_k)- F(X_k))( 2\nabla G(\theta_j ) + (T(X_k) - \nabla A(\theta_j))(G(\theta_j)- F(X_k))) \right] $$
     
      $$\leq E_{\theta_j} \left[(G(\theta_k)- F(X_k))^2( 2 v^T \nabla G(\theta_j ) + v^T(T(X_k) - \nabla A(\theta_j))(G(\theta_j)- F(X_k)))^2 \right]$$
      
      $$\leq C^2 E_{\theta_j} \left[( 2 v^T \nabla G(\theta_j ) + v^T (T(X_k) - \nabla A(\theta_j))(G(\theta_j)- F(X_k)))^2 \right]$$
      
      $$\leq C^2 [( 4 [v^T \nabla G(\theta_j )]^2 + $$
      $$E_{\theta_j} [ v^T (T(X_k) - \nabla A(\theta_j))(T(X_k) - \nabla A(\theta_j))^T v (G(\theta_j)- F(X_k))^2 + $$
      $$4 (G(\theta_j)- F(X_k) v^T \nabla G(\theta_j )  (T(X_k) - \nabla A(\theta_j))^T v]]$$
      
      $$ \leq 4C^2[c^T \nabla G(\theta_j)]^2 + C^T v^T I v + 4 C^3 |v^T \nabla G(\theta_j)|\sqrt{v^TIv} $$
      
      since by Jensen's inequality, we have 
      
      $$E[|(T(X) - \nabla A(\theta_j))^^T v|] \leq \sqrt{E|(T(X) - \nabla A(\theta_j)^T v|^2} = \sqrt{v^T I v}.$$
      
      Our final upper bound expression, collecting terms, is
      
      $$Var(v^T (MSE_estimate_k) \leq C^2 \left[C\sqrt{v^T I v} + 2 |v^T \nabla G(\theta_j)| \right]^2$$
      
      \item Hession upper bound for MSE: we have
      
      $$\nabla^2 f = \int (F(X) - G(\theta))^2 \nabla ^2 dP_{\theta}(X) - $$
      $$ \int 4 (F(X) - G(\theta))(\nabla G(\theta)) \nabla dP_{\theta}(X) -$$
      $$ \int 2 [(F(X) - G(\theta))\nabla^2 G(\theta) - \nabla G(\theta)^2] dP_{\theta}(X)$$
      
      Evaluating the gradient and Hessian, we get:
      
       $$\nabla^2 f = \int (F(X) - G(\theta))^2 [(T(X) - \nabla A(\theta))(T(X) - \nabla A(\theta))^T - \nabla^2 A(\theta)] dP_{\theta}(X) - $$
      $$ 4\int  (F(X) - G(\theta))(\nabla G(\theta)) [T(X) - \nabla A(\theta)] dP_{\theta}(X) -$$
      $$ \int 2 [(F(X) - G(\theta))\nabla^2 G(\theta) - \nabla G(\theta)^2] dP_{\theta}(X)$$
      
      Now, we shall introduce some bounds. If we assume 
      
      $$|F(X) - G(
      \theta)| < C$$ and multiply through by $v^T$ on the left and $v$ on the right, then we get 
      
      $$v^T \nabla^2 f v \leq C^2\int  [v^T(T(X) - \nabla A(\theta))(T(X) - \nabla A(\theta))^T v dP_{\theta}(X + C^2 \nabla^2 A(\theta)]  + $$
      $$ 4 C \int  |v^T \nabla G(\theta)| |(T(X) + \nabla A(\theta) )v| dP_{\theta}(X) + $$
      $$ 2 \int [(F(X) - G(\theta))v^T \nabla^2 G(\theta) v - v^T \nabla G(\theta)^2 v] dP_{\theta}(X)$$
      
      Resulting in
      
      $$v^T \nabla^2 f v \leq C^2 v^T I v + C^2 v^T I v + 4C |v^T \nabla G(\theta)|\sqrt{v^T I v} + 2C | v^T \nabla^2 G(\theta)v| + 2 [\nabla G(\theta)v]^2 $$.
      
      which for some examples of interest is convex in v: noting that the product of two convex monotone functions is convex, so the middle term is convex. 
      
      In full generality the $|v^T \nabla^2 G(\theta )v|$ could raise issues, but if $G$ is a "diagonal" / element-wise operator on $\theta$ such as the inverse logit, then the result will always be a sum of squares in $v_i$. Thus it suffices to check this term at every corner to arrive at a valid upper bound. The equation we need is:
      
      $$\frac{1}{2} v^T [\nabla^2 f] v \leq C^T c^T I v + 2 C| v^T \nabla G(\theta) | \sqrt{v^T I v} + C|v^T \nabla^2 G(\theta) v| + [\nabla G(\theta) v]^2 $$
      
    
\end{enumerate}

\end{subsection}
%%% END: LEGACY %%%

\subsubsection{Mike's note to self: should improve ALL of the notation for stopping times. i.e. "tau-max" is kinda lame, we can find better notation. also, we may literally want to replace it in the proof with a better martingale argument, so there's that too..}

\subsubsection{Ignore the section below for now}
In Section X we discussed hypotheses tests of interest. For estimation, there are several related quantities of interest for bias evaluation:
\begin{enumerate}
    \item $p_i$
    \item $\theta_i$
    \item $p_* - p_0$
    \item $\theta_* - \theta_0$
\end{enumerate}

Let us consider the most difficult case, estimating $p_* - p_0$. To begin, we can start by breaking this up into $$Bias = Bias_1 + Bias_2 = (p_1 - p_0)\mathbbm{1}\{x_{11} \geq x_{21}  \} + (p_2 - p_0)\mathbbm{1}\{x_{11} < x_{21}\}$$ and then try to estimate these quantities separately.

There are various estimators we could consider using. For simplicity, we shall use the MLE; one could also use a bias-corrected or Bayesian estimator here, with essentially no changes.

Let's consider the first term: we are interested in evaluating:

$$Bias_1(\theta) := E_{\theta}[ \left[ \hat{p_1} - \hat{p_0} - (p_1 - p_0) \right] \mathbbm{x_{11} \geq x_{21}}] = \int \limits_{\Omega} \left[\hat{p_1} - \hat{p_0} - p_1 + p_0 \right] \mathbbm{1}\{x_{11} < x_{21}\} P_{\theta}(X) dX $$

where $X$ is the uniform measure on the space of possible datasets (is this well defined? come back to check this). We may take a derivative, yielding

$$\nabla Bias_1(\cdot) = -\nabla( Pr_{x_{11} < x_{21}}(p_1 - p_0))(\cdot) + \int \hat{p_1} - \hat{p_0} \mathbbm{1}\{x_{11} < x_{21}\} (y - \mu) P_{\theta}(X) dX $$

where $y$ and $\mu$ refer back to the notation of an earlier section...

.........


..........

.........

We shall offer methods which allow us to both assess and tune the Family-Wise Error Rate for designs.

We will also show how, for a selection design, one may use this methods to give frequentist inference on the arm which is selected



%https://docs.google.com/document/d/1fi4YvMy6ArpUDdkSrgkR_XCO1Kx8OW7ct659_L56jqU/edit
\fi
%%% END REMOVE %%%

\section{Description of Examples and Content (Write Last) }

We will demonstrate our simulation-based techniques on three key examples: 
\begin{enumerate}
\item a simplified Phase II/III selection design
\item a logrank test between treatment and control
\item a Bayesian basket trial considered by the classic paper [cite Berry paper 2013].
\end{enumerate}
In each case we will discuss issues posed by the trial design, present Type I Error profile visuals, and highlight the solutions offered by our software. In example (1), we discuss family-wise error rates, tuning designs to stay under a family-wise error rate budget, Bias and Mean Squared Error of bounded estimators, and compare performance to a closure-based rule. In example (2), we discuss outcome distributions, crossing survival curves, and show various distributional families against which Type I Error protection can be demonstrated: exponential, gamma, and gamma hazard. We discuss complexities of the null hypothesis region. In example (3), we use methods for rapid Bayesian computation, showing that non-MCMC methods can perform Bayesian analyses such as those done in [Berry Paper] quickly and without compromising analysis quality, and give comprehensives profile of both the Type I Error and FDR. Our simulation framework ensures that Type I Error can still be provably controlled, even if the posterior calculations are inaccurate or incorrect. We first present Example (1) in Section X. Then, in Section X, we demonstrate how our mathematical framework models this example. In Section X, we ...


\section{Example: A Simplified Phase II/III Selection Trial}

 The trial begins with a control arm $A_0$ and two treatment arms $A_1$ and $A_2$. 
 Each arm is assigned 50 patients to start. 
 After we observe outcomes for all of these patients, 
 the first analysis is triggered and a decision will be made between $A_1$ and $A_2$: 
 we drop the arm with fewer successes, keeping $A_1$ in the event of a tie. 
 Then, the selected treatment arm and the control arm receive 200 further patients. 
 The total number of patients is thus 250.  
 After observing all outcomes, we perform a hypothesis test 
 comparing the selected treatment to control. 
 We shall consider the most naive of tests for comparing these arms, 
 based on the two-sample z-statistic, given by

\[
    Z := \frac{\hat{p_*} - \hat{p_0}}{\sqrt{\frac{\hat{p_*}(1 - \hat{p_*})}{n_*} + \frac{\hat{p_0}(1 - \hat{p_0})}{n_0} }}
\]
where $\hat{p_*}$ is the proportion of successes observed in the selected treatment arm 
and $\hat{p_0}$ is the proportion of successes in the control arm. 
We shall declare success for the chosen arm $A_*$ if $Z > 1.96$,
with the intention of controlling the Type I Error at level $\alpha = 0.025$.
It is well-known, however, that the Type I Error for this test is greatly inflated 
due to the selection in the first interim 
(noting that $\hat{p_i}$ is computed using data from both stages). 
Our framework offers rigorous mechanisms to study and correct for this inflation (\todojames{Section X}). 
We also offer tight bounds with simulation-based proof on the Type I Error 
(and power) as functions over compact multi-dimensional regions 
of the null hypothesis space (\todojames{Section X}),
estimation and corrections for bias (\todojames{Section X}),
and confidence intervals (\todojames{Section X}) \todojames{omit?}. 
We demonstrate the results in the following \todojames{subsections X-Z}.

\subsection{Type I Error}

The parameters in our setup are $(p_0, p_1, p_2)$, 
which are the true probability of success for a patient in arms $A_0, A_1, A_2$, respectively. 
We shall consider the Type I Error of the trial as a function of these parameters. 
We note in passing that in general, our methodology naturally carries over 
to studying power as well.
\todojames{Section X} discusses how we can construct an upper bound on the Type I Error 
as a function of $(p_0, p_1, p_2)$, with a pointwise confidence guarantee, i.e.
\begin{align*}
    \sup\limits_{\theta \in \Theta_0}
    \prob\br{{\hat{U}(\theta) < f(\theta)}} \leq \delta
\end{align*}
where $\Theta_0$ is a compact subspace of the null-hypothesis space,
$\theta := (p_0,p_1,p_2)$,
$\hat{U}(\theta)$ denotes the upper bound estimate of the Type I Error at $\theta$,
and $f(\theta)$ denotes the true Type I Error at $\theta$.
For this study, we fixed $\delta=0.025$ to achieve a 97.5\% confidence
and the critical threshold to be $1.96$ as before.
Since a three-dimensional surface is difficult to visualize, 
we instead present two-dimensional slices of the upper bound surface determined 
by fixing $p_0$ at \todojames{$0.2, 0.5, 0.8$}.

[figure 1] 
[figure 2]
[figure 3]

It is clear from Figures~\todojames{ref} that the Type I Error upper bound 
is not fully under $\alpha = 0.025$.
While this does not disprove that the true Type I Error 
is not controlled at level $\alpha$,
it, nonetheless, suggests that it is inflated since $\hat{U}$ is a tight upper bound.
Fortunately, Sklar proposes a technique 
for tuning the test's critical threshold 
to provably control the Type I Error (with $1-\delta$ confidence) 
by choosing a threshold
that controls the upper bound to be under $\alpha$~\cite{sklar:2022}.
We direct the readers to \todojames{Appendix X} 
for the proof and further details.

The optimal critical threshold tightly achieves level $\alpha$ for the upper bound.
Note that we still preserve the $1-\delta$ confidence of the upper bound
even after selecting the optimal critical threshold.
We show the Type I Error upper bound on the same set of slices
by fixing $p_0$ at \todojames{0.2, 0.5, 0.8}, but using the selected critical threshold:

[figure 9].

\subsection{Bias and Variance of Estimators}

For FDA submissions, it may be necessary in addition to give estimates of effect sizes, with an assessment of their bias and variance, and confidence intervals for the effects.

We can give an upper and lower bounding profile of the bias of the MLE. Here, we show this over the slice given by $p_0 = 0.5$:

[lower bound for bias of $\hat{p}_1$, as a function of $p_1, p_2$]

[upper bound for bias of $\hat{p}_1$, as a function of $p_1, p_2$]

These bias methods can also be applied to an estimate given by, for example, the posterior mean of a beta-binomial model. The method describe herein applies to general bounded estimators, where upper and lower bounds on the estimator are known.

We can also give the bias of the estimate \textit{of the selected treatment arm}, noting that its identity is random. Again, taking a slice at $p_0 = 0.5$:

[lower bound for bias of $MLE_{selected} - MLE_0$, as a function of $p_1, p_2$]

[upper bound for bias of $MLE_{selected} - MLE_0$, as a function of $p_1, p_2$]

[figure 10]

We are also able to estimate the variance of this quantity:

[lower bound for variance of $MLE_{selected} - MLE_0$, as a function of $p_1, p_2$, on slice $p_0 = .5$]

[upper bound for variance of $MLE_{selected} - MLE_0$, as a function of $p_1, p_2$, on slice $p_0 = .5$]

See Section X for further details.

We also present here the bias profile of using a Bayesian estimator instead:

%\subsection{Confidence Intervals}

%Let us assume we finish the trial with the following table of outcomes:

%[Table 1]

%Then, we would have the following 95\% confidence regions:

%[confidence plots for arms 1, 2, 3]

%We may also wish for a confidence bound on the selected arm parameter.

%[confidence bound for the selected arm]

%Or, for a confidence bound on the difference of the parameter of the selected treatment arm and control arm.

%[confidence plot for the selected arm minus control]

%We can construct this by breaking up the selection event, to ensure that our confidence procedure has under 2.5\% Type I Error combined. Here is the Type I Error expenditure corresponding to selection of Arm 1.
%[figure]
%Here is the Type I Error Type I Error expenditure for arm 2.
%[figure]

%The derivation of these confidence intervals is covered in Section X. They are based on inverting a tuned test, similar to but slightly more difficult than the material in Section X.


%\subsection{Re-design}

%We can also consider the possibility of changing the design mid-course. Let us say that the outcomes are

%[Table 2]

%and instead of moving directly to Phase III, we decide to extend the Phase II by dropping arm $A_2$ and adding a new arm $A_3$.

%Then the remaining Type I Error in the trial, also known as the conditional Type I Error, can be upper bounded. Here is a visual on the slice $p_0 = 0.5$:

%[figure 11].

%Noting that we did not use some of the Type I Error at the beginning, we can instead use this extra slack during re-design. Here is the upper bound with slack, over the slices of $p_0 = 0.5$:)

%[figure 12]

%\subsection{Generalizations}
%A final note: to keep this example relatively simple, we chose to omit early stopping for success or futility and censoring. But, we should note that extending these methods to these cases (assuming any censoring is non-informative) merely requires altering the simulations without further changes to the analysis code.) The analysis is flexible, if computation permits.

%\section{CUT! Basics of Software Structure and how to run the analysis in the previous section (James)}

%Here, perhaps we can give a tutorial so that one could replicate the above analysis, or change some aspects of the simulation, staying within the binomial family.

%We should try to include complete code chunks to replicate our whole analysis in section 3

\section{Example (2): log-rank survival with parametrized outcomes}

\subsection{the design: define the outcome space, log-rank test}

The log-rank test is one of the most commonly used survival analysis techniques for comparing treatment against control. The classical approach is to control Type I Error in asymptotic fashion, using a normal approximation to the test statistic under the null hypothesis of zero treatment effect.

Our simulation techniques appear at first to have the downside of needing a particular parametrized family to simulate from. In actuality, this may be no downside at all, for two reasons:

\begin{itemize}

\item since in cases where a standard normal approximation holds, a Brownian approximation typically also applies to the test statistics of the parametrized family. Thus, even if the parametrized family is not the correct model per se, protecting against Type I Error within the parametrized model class may succeed in protecting against Type I Error for general zero-effect or harmful treatments. However, this is a nuanced argument and the property is not fully general; we leave its further exposition to future work.]

\item In some specific cases, protecting the Type I Error against parametrized families can, by force, imply protection over large classes of supposedly non-parametric or semi-parametric models. For example: consider the set of proportional hazards models, which we shall define according to any functions $\lambda_T(\cdot)$ and $\lambda_C(\cdot)$ such to the constraint that $\lambda_T(t)/\lambda_T(t) = C$, a constant hazard ratio.
Let us consider the set of such censored models as defined by $PH(\lambda_T(t) , \lambda_C(t), C)$ where $C >0$, possibly infinity, is a known administrative censoring time common to all patients. Now, compare this set to $EXP(\lambda_T,\lambda_C, D)$ which represents performing a rank-based test on exponential outcomes, censored at time $D > 0$, possibly $D = \infty$. It is clear that $EXP$ is contained in $PH$; but it is also true that $PH$ covers $EXP$, as long as the statistical test of interest is based exclusively on the ranks of observed failure times. The reason for this is that any model in $EXP$ can be converted into $PH$ via a time dilation (i.e. a monotone function $R^+ \to R^+$ which takes $t$ to $t'$) such that in the new time unit, the hazard rate is constant. This transformation may change the perceived censoring time but does not change the ranks, hence full Type I Error control over the class $EXP$ implies full Type I Error control over class $PH$ for rank-based tests such as the log-rank test.

\item Our methods do offer a corresponding upside: that of allowing protection against Type I Error within large and believable classes of models where standard methods do not have traction, such as parametrized models which do not obey proportional hazards and may have crossing curves.
\end{itemize}

In particular, we will study outcomes $(y_t, y_c)$ of the following types: 


\begin{enumerate}
    \item $$y_T \sim Exponential(\lambda_T); y_C \sim Exponential(\lambda_C)$$
    \item $$y_T \sim Gamma(\alpha_T, \beta_T) ; y_C \sim Gamma(\alpha_C, \beta_C)$$
    \item $$\lambda_T \sim Gamma(\alpha_T, \beta_T) ; \lambda_C \sim Gamma(\alpha_C, \beta_C)$$
\end{enumerate}

In model (2), the outcomes are distributed as Exponential
In model (2), the outcomes are distributed as Gamma. (Note that this model class contains the class of exponential outcomes, which models the hazard $\lambda_C$ as constant.) The final model (3) is technically a sort of frailty model, where each patient has their own unique hazard rate $lambda_i$, drawn from the corresponding treatment or control distribution - both models corresponding to draws from a gamma distribution. Model (3), as well, is in a sense an enlargement of Model (1), in the sense that by sending $\alpha , \beta \to \infty$ while keeping their proportional fixed, we approach the constant hazard model with exponential outcomes.

In the next section, we discuss the null hypothesis regions of these models

\subsection{Null hypothesis regions and discuss curve-crossing issues}

In Model (1), we may simply say that if $\lambda_T \geq \lambda_C$, the risk is lower under control, thus the control is preferred and we are in the null hypothesis.

[Insert 2-D plot]

But in general when survival curves cross [as may occur in Models (2) and (3)], the story is not so simple. 

One simple was to approach the issue is to split the problem into 3 regions: Clear null, curve-cross (gray), and clear alternative.

[I'm not sure how best to present this, i.e. along which dimensions, but we should definitely present some sort of visual here!]

We may, however, be able to take a stronger position that simply deferring in the event of crossing curves. We could, for example, compare the expected survival times under model (2).

[insert the equations and a visual for this; probably fix the control distribution as exponential, and draw this plot in terms of the treatment alpha and eta]

Or, we can take inspiration from RMST analysis, and

\subsection{define sets of mathematical models with which we could compare to}

\subsection{show plots of Type I Error}

Alex had a great idea: in multiple dimensions, try to maximize the FWER along the unseen dimensions

\subsection{evaluate relevant bounds from section 4}

\section{Example (3): Bayesian Basket Trial}

\subsection{Summarize the setting from Berry 2013}

\subsection{Discuss our replacements for MCMC, and compare our graphics to what Berry et al. gave}

\subsection{Provide Comprehensive Visuals: Type I Error and FDR}

\subsection{FDR Methodology}

\subsection{A Remark On Monotone Tuning for Adaptive Trials}

For the above proofs to apply, we require that if $\lambda_1 < \lambda_2$ the rejection set under threshold $\lambda_1$ must be strictly contained in the rejection set under $\lambda_2$. However in some problems with multiple arms and multiple stages of analysis, such as in [Lei example] one might be tempted to index the tuning rule by, for example, the posterior probability of success. However, this choice can break the containment property of of rejection set, since changing the threshold to reject one arm at an earlier interim could hypothetically cause another arm not to be rejected later on.

In practice, if there is a final analysis, one should usually be able to set up the simulations with sufficient accuracy so that tuning is effectively restricted to the final stage, barring some catastrophe of chance in the simulation RNG where the previous analyses consume the full Type I Error budget. The odds of such a catastrophe can be driven arbitrarily low by performing enough simulations, if the design is calibrated properly.

But should such a catastrophe happen, then what? For the sake of giving a fully robust theoretical fallback, one could define the tuning process with respect to a total ordering of the sample space, such as Siegmund's ordering. [Find reference from my thesis]. This ordering takes the time $t$ and a rejection statistic $S_t$ such that smaller values of $S_t$ favor rejection. Siegmund's ordering is then the lexicographic ordering on the pair $(t,S_t)$, so that earlier times are generally preferred for rejection. Tuning with this setup gives the fallback of effectively removing analyses from the back to the front until control is established.

In practice, should this occur, most likely a mistake has been made and a re-design should be performed. Tuning for re-designs will be a topic of future work.

\subsection{Remarks on Conservatism / Power Loss of Tuning}

In this subsection we walk through some formulaic approximations to the Type I Error and power lost due to simulation tuning. Our goal will be to build intuition for how many simulations are necessary to run.

Consider for simplicity a single ``worst case" hypothesis point, upon which the methods of Section X are applied. (This point could be the only one that matters if the Type I Error function is very peaked, so that the high point is almost certain to yield the maximum Type I Error in simulations.)

Let us assume an overall Type I Error guarantee of 2.5\% is sought; and continuous simulation extension costs .1\%, leaving 2.4\% remaining for Type I Error at the point itself. We remark that this .1\% should not be fully accounted as ``lost to conservatism", noting that the Type I Error function could indeed be increasing at a rate which nearly matches the CSE bound. Include here some Figure X, one of the ones James has recently created, which shows how closely our bound tracks.

We perform $n = 10000$ Monte Carlo simulations at this point. On average, at the true ``optimum" point $\lambda'$, the rate of simulations yielding a positive result will be 2.4\%. The number of simulations to estimate Type I Error as this point is therefore about Poisson(240), with a standard deviation of about $\sqrt{240}$. Then, roughly speaking, noting that the selected $\lambda^*$ is the value such that $\hat{f_{\lambda^*} = 2.4\%}$ (up to some offset on scale 1/n due to discretization) we should expect the Type I Error achieved by $\lambda^*$ to have $E[f_{\lambda^*}] = 2.4\% + O(1/n)$, and $SD[f_{\lambda^*}] \approx \sqrt{2.4\% / n} \approx .15\% $. (To establish this approximation more rigorously, one could use the beta distribution, or appeal to a logic similar to the Wald confidence interval for the binomial.)

So there is negligible lost Type I Error on average, on order $O(1/n)$, and a larger degree of variability on the order $O(1/\sqrt{n})$. How does this translate to lost power? If the design is calibrated roughly to be like a 1-sided z-test ``80\% Power, 2.5\% Type I Error", we can approximate the marginal value of gained or lost Type I Error with the formula

$$\frac{\phi(\Phi^{-1}(.8))}{\phi(\Phi^{-1}(.975))} \approx 4.79$$

In this approximation, gains and losses to the Type I Error would translate with a multiplicative leverage of roughly 4.8 at the 80\%-power implied alternative. The dominant term then the excess conservatism due to CSE bounding, which is somewhere between $0$ and $.1\%$, which translates to a loss of about between $0$ and $.5\%$ power at the implied 80\%-power alternative. The other terms are negligible in size - the $O(1/n)$ loss due to discretization is minimal, and variability approximately leads to equal gain and loss on both sides and can be ignored (although for smaller values of $n$, the variability of $f_{\lambda^*}$ may become relevant and require further corrections for accuracy.)

But now we can ask: what would happen if there were $K$ worst-case points with borderline Type I Error, not just 1? For one thing, the Type I Error function is continuous and often quite flat across nuisance dimensions; and, if there are symmetries in the design which have not been accounted for, the ``worst case point" may actually be a set of distant but symmetric points.

In this case, with the settings described above, each worst-case point $\theta^i$ individually would have the tuned net performance $f_{\lambda^{i*}}$ which is approximately normal, with:

$E[f_{\lambda^{i*}}] = 2.4\% + O(1/n)$, and $SD[f_{\lambda^{i*}}] \approx \sqrt{2.4\% / n} \approx .15\%$

but because we take a minimum of the tuning thresholds in Section X, the minimum of these random variables is likely to have expectation significantly below $2.4\%$. If the simulation estimates at these points are not correlated, then the expected conservativeness is approximately $SD[f_{\lambda^*}^i] * E[M]$ where $M$ is the minimum of $K$ i.i.d. standard normal R.V.'s. For 2 points, $E[M]=1/2$ and the expected contribution to Type I Error loss is therefore $.15 \% /2\ = .075\%$. The resulting net loss to power at the $80\%$ alternative is between $(.075\%)* 4.8 \approx .4\%$
and
$(.1\% + .075\%)* 4.8 \approx 1.2\%$, depending on how much of the CSE bound should be accounted as excess loss.

In practice, how should one estimate $E[M]$ when the number of such near-worst-case points is not strictly defined or known? We note that if there are $K$ correlated Gaussians each with mean $\mu$ and variance $\sigma^2$, the expectation of the maximum is

$$E[M]\leq \sigma \sqrt{2\log K}$$

So what is $K$, the plausible number of competitors for the worst case point? One option here, using pilot simulations, is to make a confidence bound and exclude all points which are significantly below the largest observed Type I Error.

\subsubsection{Improved Stopping Criteria via the Bootstrap}

When performing a series of pilot simulations, the above may not be so helpful; it assumes the means of these candidate points are all the same, that they have roughly the same number of simulations, and for tightness it is required that the simulation estimates are approximately independent. None of these things are true in our implementation of adaptive gridding.

So then what? We propose (without proof) to do a type of bootstrapping, where as a stand-in for the population ``optimal test" Type I Error surface 

$$f_{\lambda^{**}}(\theta),$$

 we use the empirical ``tuned test" contour

$$\hat{f}_{\lambda^*}(\theta)$$

noting that both of these will be maximized at close to the target value $\alpha = 2.5\%$.

Then, in the process of computing the empirical tuned test, we can compute e.g. 10 resamples of the data with replacement, and for each of them compute

$$\hat{\hat{f}}_{\lambda^{*b}}^b(\theta)$$

for $b = 0,1, \ldots, B$.

Then, to understand how conservative on-average our current choice of sim-sizes is making things, we are interested in the ``bias surface":

$$E[\hat{f}_{\lambda^*}(\theta) -
f_{\lambda^{**}}(\theta)]$$

A natural point at which to look at this surface, though not the only one to consider, is the worst-case largest value.

As a means of estimating this, we will plug in $\hat{f}_{\lambda}$ in place of $f_{\lambda}(\theta)]$, and to get a distributional understanding, plug in $\hat{\hat{f}}^b_{\lambda^{*b}}$ in place of $\hat{f}_{\lambda^*}$.

[Note for Ben: when we use the actual sample as "ground truth", I think the ideal way of estimating would be to allow the value of lambda to shift, and take on those r different values! I know that this would cause problems for concurrency, though...]

Thus our estimate of the bias function is

$$\frac{1}{B}\sum_{b=1}^{B} \hat{\hat{f}}^b_{\lambda^{*b}}(\theta) - \hat{f}_{\lambda^{*}}(\theta)$$

%\section{OLD VERSION: Continuous Simulation Extension (CSE): the z-test}
%To give a demonstration of continuous simulation extension (CSE) in a familiar setting, we analyze the Type I Error of the one-sided z-test, with critical value set to 1.96. That is, our data will be a single draw $Z \sim N(\mu, 1)$, where $\mu$ is a scalar unknown parameter, the null hypothesis is $H_0: \mu \leq 0$, and our test is given by the rule: ``reject if $Z > 1.96$".
%The true power curve for this z-test hits approximately 2.5\% at $\mu = 0$, and it is smaller everywhere to the left (see the dotted line in Figure 1).
%\includegraphics[width = 6cm, height = 6cm]{power of ztest.png}
%The z-test is typically analyzed by integrating the normal curve. But this mathematical analysis can break down for modern complex trial designs, where normal approximation arguments may be too loose for reasons including:
%\begin{enumerate}
%\item Slow central limit convergence in finite samples.
%\item Non-Gaussian limit behavior due to adaptive sampling. The resulting limiting distributions are also usually non-pivotal, which causes the bootstrap to fail \cite{chuang1998resampling}.
%\item Other mathematical migraines caused by complex randomization plans or multiple hypothesis testing.
%\end{enumerate}
%So, instead of the analytic approach, we will control Type I error with simulations combined with CSE. Our end goal is to deliver the confidence bands on Type I Error in Figure \ref{uandl} by simulating over the null hypothesis space $\mu \leq 0$. 
%\begin{figure}
%\includegraphics[width = 8cm]{power-ztest.pdf}
% add something here with quadratic bounds that has different components visible
%\caption{Upper and lower bounds on the Type I Error of the z-test, as a function of the unknown true mean $\mu$}
%\label{uandl}
%\end{figure}
%Our bounds are a pair of functions $l(\theta), u(\theta)$ with the following key properties:
%$$\forall \theta \in \Theta_0, P(f(\theta) < l(\theta)) < \delta/2$$
%$$\forall \theta \in \Theta_0, P(f(\theta) > u(\theta)) < \delta/2$$
%Thus at each value of $\theta$, the pair $(l(\theta), u(\theta))$ is a valid $1-\delta$ confidence interval about the true Type I Error. One-sided problems such as a regulatory requirements for Type I Error can be easily handled by setting $l= -\infty$ and using only the upper bound $u$. 
%Before we describe how to construct these bounds, we will discuss potential concerns about such intervals:
%\begin{enumerate}
%    \item Our bounds only cover the %space $\Theta_0$ near where we have taken simulations.
%    \item Our bounds may be undesirably conservative.
%    \item A 1-$\delta$ confidence interval is still not a certainty.
%    \item We may fail to establish a guarantee at a fixed desired level $\alpha$. For example, observe that in Figure X, $u(\theta)$ is larger than 5\% almost everywhere.
%\end{enumerate}
%Fortunately, all of these concerns can be addressed. Issues 1-3 can be addressed with increasing computation: Issue 1, by expanding the space $\Theta_0$. Issue 2, by performing more simulations on a finer grid, so that the upper bound becomes tight. Issue 3, by taking $\delta$ very small, and adding more simulations to compensate for the increased confidence width. %We also use adaptive gridding methods to reduce the grid density and the number of simulation. % Let's skip adagrid for this paper
%Furthermore, we also note that for issue 1, sometimes there are analytic arguments which can provide coverage over the remainder of the space\footnote{In fact, loose analytic tail bounds can dovetail very well with CSE, as they cover each others' weaknesses. CSE can control Type I Error sharply in locations where it is largest; and for the rest of the space, loose approximations are affordable where the Type I Error is small.}.
%Finally, the methods in Section X will
%provide a solution to issues 3 and 4, and may also be less conservative. 
%There, we introduce a tuning approach that can provide a true 2.5\% guarantee, at the cost of shifting our critical value. This shift is conservative on average, the power lost to conservatism is reduced with more simulations and a denser simulation grid: see Figure \ref{cost-tuning-fig}. %(resulting in mild conservativeness on average).
%With these concerns addressed, we now flesh out the key technical ideas for constructing $u$.

%\footnote{the first issue of failing with some small probability, can be traded off against the conservativeness of width by choice of delta; the second is ameliorated by doing more simulations at a tighter grid, and the third issue can be tackled by widening the simulation grid to all plausible values. loose analytic proofs may also be sufficient to truly complete the argument outside of a bounded range; we may not need to be particularly tight, far away from the null boundary.}

%\begin{figure}
%\includegraphics[width=8cm]{z-test-cost.pdf}
%\caption{Needs to be re-implemented for ODI! A plot of the average conservativeness of the tuned z-test, under a range of different proof-by-simulation setups. In this plot, a y-value of .4\% indicates that the average Type I Error is 2.5\% - .4\% = 2.1\%. With larger N and a denser grid, the cost approaches zero and the tuned rule becomes tight to the target 2.5\%.}
%\label{cost-tuning-fig}
%\end{figure}

%\subsection{Task A: Continuous Simulation Extension (CSE) for Descriptive Bounds}
%\label{ssec:ztest-describe-task}

%\begin{figure}
%\includegraphics[width = 12cm]{ztest-four-panels.pdf}

%\caption{Throughout all panels, the Type I Error curve as a function of the unknown parameter $\mu$ is plotted as the dotted red line. A) The dotted red line is the true Type I Error curve. The error bars show simulated Type I Error and confidence intervals at $\mu =-0.75$ and $\mu = -0.25$. The dotted blue line shows a Type I Error curve that is plausible given only the two points of information. B) Confidence bounds on the gradient are constructed from simulations and used to approximate the change in Type I Error near the simulation points. C) The 0th order confidence intervals (the error bars), the combined 0th order and 1st order confidence intervals (the shaded blue regions), and the 0th order plus first order plus 2nd order upper bounds (dotted black lines). D) A demonstration of bound convergence as both N, the number of $\mu_i$ values, and S, the number of simulations, increase. The blue line uses N = 18 and S = 106 resulting in a tight fit to the true Type I Error curve.}
%\end{figure}

%We begin with standard Monte Carlo on a grid of points - in this case, $\theta_i = \{-.75, -.25\}$. Denote the grid $\theta_i \in \Theta_0$, and repeatedly simulate the Type I Error at those points. With these replications, we can construct Clopper-Pearson confidence intervals
%\includegraphics[]{basic_conf.pdf}
%which give a 95\% confidence bound on the Type I Error function at each $\theta_i$. But what about the space in between? In reality the true Type I Error function, represented by the red dotted line in Figure 2A, is well-behaved and controls the Type I Error at the 2.5\% level. But to establish this, one must rule out ``wiggly" functions like the blue dotted line, which pass through the Type I Error confidence intervals yet still exceed 2.5\% in between. How can we achieve this using only simulations at $\theta_i$?

%\includegraphics[height = 6cm]{Screen Shot 2022-08-11 at 4.25.11 AM.png}

%To resolve this problem, we perform a Taylor expansion of the Type I Error function, $f(\theta)$, at the simulation points. For any point $\theta'$ with some nearby $\theta_i$, Taylor's theorem tells us that we can describe the Type I Error as:

%$$f(\theta') = f(\theta_i) + (\theta' - \theta_i) f'(\theta_i) + \frac{1}{2}(\theta'-\theta_i)^2 f''(\theta'')$$

%where $\theta''$ is some point in $[\theta_i, \theta']$. Note that for the first term $f(\theta_i)$, which we shall call ``0th order" as it takes no derivative of $f$, we can construct a $1-\delta$ confidence bound by using the simulated rejections under $\theta_i$, using Clopper-Pearson. For the second term $(\theta' - \theta) f'(\theta_i)$, which we call the ``1st-order" term as it involves $f'$, we begin by constructing a confidence interval for the first derivative $f'(\theta_i)$. In Appendix section X, we demonstrate that $\frac{1}{N} \sum \limits_{j=1}^N F_j (Z_j - \mu)$ is an unbiased estimator of $f'(\theta_i)$. As a result, we can use Chebyshev's inequality to derive a confidence bound on $f'(\theta_i)$:

%$$
%Pr\left( |f'(\theta_i) - \frac{1}{N} \sum \limits_{j=1}^N F_j (Z_j - \mu)| \leq \sqrt{\frac{1}{N\delta}} \right) \geq 1- \delta.
%$$

%where $F_j = 1$ if simulation $j$ is a false rejection and otherwise  $F_j = 0$, and $Z_j$ is the drawn value of $Z$ in simulation $j$. We may extend this confidence bound to a bound on the relevant Taylor term $(\theta' - \theta_i)f'(\theta_i)$ simplying by multiplying by $(\theta' - \theta_i)$. Thus, as we change $\theta'$, the resulting band will be linear in $|\theta' - \theta_i|$. See Figure 2B, where the confidence bands have been broken into regions according to which $\theta_i$ is closest.
%\includegraphics[]{first_deriv.pdf}

%Finally, for the last Taylor term, techniques from Appendix Section X imply that any hypothesis test on a 1-dimensional standard Gaussian, the Type I Error must satisfy $|f''| \leq 1$ uniformly. Therefore: $$ -\frac{1}{2}(\theta'-\theta_i)^2 \leq \frac{1}{2}(\theta'-\theta_i)^2 f'' \leq \frac{1}{2}(\theta'-\theta_i)^2$$. 

%This term yields a parabolic penalty away from each $\theta_i$. Summing together these 3 pieces in the Taylor Expansion, we arrive at a Figure 2C's joint upper bound for $f(\theta)$, which holds with $1-2\delta$ pointwise confidence.
%\includegraphics[height = 6cm]{final_conf.pdf}
%Note that these bounds far exceed 2.5\% in some places, which is undesirable. We can tighten the bound by increasing the number of gridding points $|\{\theta_i\}|$. By tightening the gridding density, we arrive at Figure 2D where we show the bound for N=2, 6, and 18 where N is the number of grid points. We also show the effect of increasing the number of simulations: the 0th and 1st order confidence intervals tighten, but the 2nd upper bound remains unchanged.

%\includegraphics[height = 6cm]{conf_bands.pdf}

%We have thus shown how to perform Task A for Type I Error for a 1-dimensional Gaussian statistics. The arguments above are generalized in Appendix Sections X - Y to handle exponential family outcomes in more than one dimension, with extensions to FDR, and bias and MSE of bounded estimators.

%\subsection{Task B: Tuning to Establish Provable Type I Error Control}
%\label{ssec:ztest-tuning-task}

%But we have not proven true control over the Type I Error at the 2.5\% level, since the bounds can still exceed 2.5\% (which does in fact occur in this seed!). Recall task B, which sought a procedure that provably controls Type I Error. To achieve this, we shall \textit{tune} the critical value.\footnote{A conceptual clarification: for task A, we take a fixed procedure, and our Type I Error bound is mildly random. For task B, it is the opposite: we seek a fixed Type I Error \textit{guarantee}, and we  achieve this pushing randomness into the design, because tuning gives a random threshold when based on simulations. Fortunately, our guarantees account for and remains valid under this randomness, assuming the user is not able to game the simulations by re-running them or choosing the seed.
%Thus, we expect this form of guarantee to be the preferred method for Phase III trials where Type I Error control is at issue. In contrast, perhaps Form A is relatively more appealing in other phases, where there may be less need for Type I Error control to drive the tuning decision.}
%In this subsection we describe key features of this approach, leaving a fuller mathematical description to Appendix C.

%Similar to the approach described in Section \ref{ssec:ztest-describe-task}, we develop a method for bounding the deviation of the Type I Error away from the simulation points. Because Task B is specific to the Type I Error and aims to bound Type I Error at a small value, we use specialized upper bounds which are more efficient in the low-Type-I-Error range than those shown in \ref{ssec:ztest-describe-task}. These new bounds are based on differential inequalities for the Type I Error - see Appendix C for full details. This ODI bound depends on the point Type I Error $f(\theta_i)$, but not the derivative $f(\theta_i)$, which makes it slightly simpler to use.

%[Create a graphic which shows the projected-forward TIE from a given point $f(\theta_0)$, given multiple `starting points' of $f(\theta_0)$. This gives us a bunch of vertically offset identical curves.
%Highlight the one which crucially hits 2.5\%!

%Caption: Figure X. Several possible upper bounds are drawn, each one of them relying on an assumed value of $f(\theta_i)$ = [point 1 , point 2, point 3, point 4.] Note that at point 3, the bound does not exceed $2.5\%$ in the range [-.5, 0].
%]

%From this, we can deduce that if our tuning \textit{procedure} were to control the TIE at less than $intercept\%$ at the point $\mu = -.25$, then Type I Error of following our tuning procedure does not exceed $2.5\%$ over the region $[-.5, 0].$

%How to establish this control at the point $\mu = -.25$? Fortunately, the naive approach works: we simulate the test statistic under 10,000 times under $\mu = -.25$, and slide the critical value until 2.5\% of those simulations reject. A more general proof is provided in Appendix C.

%To achieve this at both $\mu = -.75.$ and $-.25$ simultaneously, we can simply perform this tuning procedure on both and then use the more conservative threshold. Similarly, with more points we would take the most conservative thresholds among all of them.

%[Create new figure!] 

%How conservative is this approach? It will depend a variety of factors, including the gridding density, number of simulations, and whether the simulations at different grid-points have been correlated by sharing RNG \footnote{As long as the simulations are independent within each grid-point, correlation across different grid-points is not a problem for the proofs and in fact is generally helpful for smoothing out estimates. Our figures all use correlated simulations.} In figure X we present the overall conservativeness of this approach, as a function of the number of data points and the number of simulations. The loss to conservatiness can be decreased toward $0$ with increasing simulation count and denser gridding.

%[create new figure! showing net overall consequence]

%[PREVIOUS CONTENT REMOVED: READER IS REFERRED TO APPENDIX C]..

\if 0
we take a grid of critical thresholds, such as $z^* \in \{1.96, 2.0, 2.04, 2.08\}$, and pick one which is more conservative than all of those whose confidence bounds exceed 2.5\% \footnote{If all of them should exceed 2.5\%, we set $z^* = \infty$ to "reject nothing" as a failsafe}. Evaluating this, we find that the worst upper confidence bound breaks 2.5\% for $z^* \in \{1.96,2.0\}$, but not for any of the larger critical values. So, we pick
$z^* = 2.04$ as a safe test threshold. Taking $z^* = 2.04$ turns out to yield a conservative true Type I Error of 2.07\%, see Figure \ref{cost-tuning-fig}.

\begin{figure}
\includegraphics[width=8cm]{tuned-ztest.pdf}
\caption{The red dashed line shows the true type I error profile given a one-sided z-test threshold of $z^* = 2.04$. The dark black lines shows the rough upper bound computed for this threshold using 9 points in $\mu \in [-1, 0]$ while the faded lines show the upper bound for the other three threshold: $z^* \in \{1.96, 2.0, 2.08\}$. }
\label{intro_tuning_fig}
\end{figure}

Results in Appendix A and C show that despite the random selection of $z^*$, $$P(\sup \limits_{\mu \in \Theta_0} TIE(z^*) > 2.5\%) < 2\delta.$$
%the probability that the maximum Type I Error under the selected $z^*$ is greater than $2.5\%$, is less than $2 \delta$.
where $TIE(z^*)$ is the Type I Error of the z-test with critical value $z^*$ chosen by this procedure. Furthermore, selecting $z^*$ in this way \footnote{Note that the choice of $z^*$ is viewed here as a random selection procedure, subject to simulation randomness, and the expected Type I Error guarantee holds with respect to the simulation randomness.} 
controls the overall average Type I Error at the level
$$E[TIE(z^*)] \leq 2.5\% + 2\delta$$

A general proof and a variety of alternative methods are given in Appendix Sections A and C. If one desires a flat 2.5\% guarantee rather than $2.5\% + 2\delta$, one can simply replace the 2.5\% tuning target used earlier with the quantity $2.5\% - 2\delta$. \qedsymbol

\fi


==> scratch.tex <==
While the Tilt-Bound is posed with parametric data,
non-parametric analysis sometimes holds.
Example~\ref{ex:non-parametric} shows an example
of applying the Tilt-Bound for testing a non-parametric model
with Gaussian additive noise.

\begin{example}[Non-parametric Model with Gaussian Noise]%
\label{ex:non-parametric}
Assume a simple non-parametric model for outcomes 
$Y = \{y_i\}$ conditioned on a (1-dimensional) covariate
$X = \{x_i\}$ for $i \in 1, \ldots, n$:
\begin{align*}
    y_i & = g(x_i) + \epsilon_i\quad 
    \\
    \epsilon_i & \sim \Normal(0,1)
\end{align*}

Consider a test of the form $F(y) := \indic\pr{y \in S}$ 
for some set $S$. 
We assume the regression function $g \in G$ is not known. Our goal is to bound over $G$ the Type I Error conditioned on the covariate vector, i.e. a bound on $f_X(g) := \EEE_{g}\br{F(Y) | X}$. We may define the metric
\begin{align*}
    d_{L^2_{X}}(a, b) 
    := 
    \pr{
        \sum\limits_{i=1}^n
        \br{a(x_i) - b(x_i)}^2
    }^{\frac{1}{2}}
\end{align*}

and aim to derive a bound valid within a $L^2_{X}$ neighborhood of some function $h$. We apply the Tilt-Bound directly. 
Conditional on $X$, the distribution of $Y$ 
is an $n$-dimensional Gaussian, 
hence an $n$-dimensional exponential family. 
The Tilt-Bound evaluates to
\begin{align}
    f_X(g) 
    &\leq 
    f_X(h)^{1-\frac{1}{q}}
    \exp\br{\frac{q-1}{2} \norm{h - g}^2_{L^2_{X}}}
    \label{eq:ex3-tilt-bound}
\end{align}

Conveniently, for $g$ in the $L^2_X$ ball of $h$ of radius $r$,
$B_{L^2_{X}}(h, r)$, 
the worst case of this bound occurs at all points on the boundary of
$B_{L^2_{X}}(h, r)$. 
As a result, CSE can be applied to bound 
$f_X(g)$ over a covering of $G$ with an 
$\epsilon$-net in $L^2_{X}$,
and using~(\ref{eq:ex3-tilt-bound}) 
to bound each $\epsilon$-ball of the covering.
\end{example}

